Who Should Review Your Proposal? Interdisciplinary Topic Path Detection for Research Proposals

The peer merit review of research proposals has been the major mechanism to decide grant awards. Nowadays, research proposals have become increasingly interdisciplinary. It has been a longstanding challenge to assign proposals to appropriate reviewers. One of the critical steps in reviewer assignment is to generate accurate interdisciplinary topic labels for proposals. Existing systems mainly collect topic labels manually reported by discipline investigators. However, such human-reported labels can be non-accurate and incomplete. What role can AI play in developing a fair and precise proposal review system? In this evidential study, we collaborate with the National Science Foundation of China to address the task of automated interdisciplinary topic path detection. For this purpose, we develop a deep Hierarchical Interdisciplinary Research Proposal Classification Network (HIRPCN). We first propose a hierarchical transformer to extract the textual semantic information of proposals. We then design an interdisciplinary graph and leverage GNNs to learn representations of each discipline in order to extract interdisciplinary knowledge. After extracting the semantic and interdisciplinary knowledge, we design a level-wise prediction component to fuse the two types of knowledge representations and detect interdisciplinary topic paths for each proposal. We conduct extensive experiments and expert evaluations on three real-world datasets to demonstrate the effectiveness of our proposed model.

==> document/abstract_old.tex <==
% 句子1：why we need proposal classification?
% 科研工作是难以离开资金支持的，为了将科研经费分配到更加合适的项目中，自然需要为项目申请书组织评议。但由于申请者与管理者都缺失对学科体系的全貌的了解，通过申请者填写来合理分配评审专家成为了一个困难的工作。为了为各领域的研究分配合适的评审专家，自然需要为这些研究划分研究主题，并通过这些主题找到评审专家。
The development of science is indispensable to the funding supply, which needs an open-court competition organized by government agencies (e.g., NSF) for every scientist between their research proposals. 
% Generally speaking, we all want our well-written research proposals to be reviewed and commented on by reviewers knowledgeable about the corresponding fields. 
Generally speaking, reviewed and commented on by reviewers knowledgeable about the corresponding fields for the research proposals is a common desire for each researcher.
% 句子2：what is proposal classification?
% 主要目的是为申请书找到最合适的相关领域，并以此为指导寻找更为合适的审稿人
Thus, it is critical to identify the correct fields a research proposal belongs to. 
% 句子3：why is your proposal classification challenging?
% 1、学科体系复杂，2、学科交叉涌现，3、学科间term形成的壁垒
% However, the complexity of the discipline system and the emergence of interdisciplinary research make it increasingly challenging to recognize the correct areas. 
However, this task is still challenging due to three reasons:
(1) The research domain is numberless. In other words, if we treat the discipline system in a flat view, the label number will be considerable.
(2) An increasing number of research proposals show interdisciplinarity. We have to find experts from one or more domains in different disciplines to evaluate their value for a fair peer-review.
(3) The research proposals consist of multiple documents containing semantic information with different meanings according to their categories.
% discipline system
% (1) From the researcher's side, it might be easy to figure out the primary discipline of their study. Still, the more fine-grained and the related interdisciplinary fields are hard to determinate. 
% number
% (2) On another side, the funding administrator might be familiar with the whole picture of the discipline system, but their effort cannot sufficient the exploding number of applications. 
% words and term
% 句子4：what is your proposed framework? framework name and framework high-level idea
% 
This paper focuses on developing a top-down architecture named Hierarchical Interdisciplinary Research Proposal Classification Network (HIRPCN) to overcome the three characteristics jointly.
% In this paper, we proposed a novel method named Hierarchical Interdisciplinary Research Proposal Classification Network (HIRPCN) to solve the dilemma. 
% Although certain prior studies focus on similar fields like text classification and hierarchical multi-label classification, there are essential differences between this task and others: 1) Each proposal should be categorized into one or more sub-disciplines, which consist of several variant-length sequences of labels; 2) The discipline system naturally exhibit the hierarchical information between the discipline and their sub-discipline; 3) Every discipline whether how fine-grained, shows a cross-disciplinary characteristic with others;  4) The research proposals contain multiple types of documents;
% 句子5：what are your technical contributions to achieve the goals of your framework?
We first use a hierarchical Transformer as a document Encoder to extract the information within the document and among each type of document. After that, we build an interdisciplinary graph and use the Graph Neural Networks to capture the representation of each prediction result. Then we design a level-wise label generation architecture to utilize the dependency information from previous prediction results for the next level's label generation.  
% 句子6：based on your framework, do you develop a demo/system/deployment/field testing?
We developed a demo\footnote{try demo at http://101.35.54.56/} based on the HIRPCN to demonstrate the attention mechanism and prediction process.
% 句子7：what are your lab experimental results and field experimental results?
The experimental results show that HIRPCN beats other baselines by utilizing these unique features. Moreover, we further visualize the attention value to prove the model behavior. The other experiments show a practical potential to employ this model on the online system.
% 句子8：what are the underlying implications/insights of your work for applied data science and real world NSF propsal assignment?? 
Besides this, by collaborating with experts from a different domain, we prove that HIRPCN can find the hidden interdisciplinary label for the research proposal, significantly improving the peer-review system and the real-world NSF proposal assignment. 



\iffalse
The development of science is indispensable to the funding supply, which needs an open-court competition organized by government agencies (e.g., NSF) for every scientist between their research proposals. 
% 背景
Generally speaking, finding the most relevant discipline for research proposals can help the funding administrator allocate the proposal to suitable experts. 
% 目的 - 找到最相关的学科能够协助基金管理者分配专家
However, due to the complexity of the discipline system and the emergence of interdisciplinary research, it becomes challenging to classify the research proposals into one or more correct fields. 
% 问题 - 由于学科体系的复杂性与交叉学科的涌现
To address that, this paper study the Interdisciplinary Research Proposal Classification (IRPC) task for the first time. We propose a model named HIRPCN. By adaptively utilizing abundant semantic information and various interdisciplinary knowledge, HIRPCN can classify the multiple type text into the most fine-grain discipline or interdiscipline in the real-world dataset. HIRPCN can also start from an expert given discipline to complete label prediction.
% In this paper, we apply 
% \note{The tech sounds naive.
% the hierarchical multi-label classification architecture and text classification technique} into the Interdisciplinary Research Proposal Classification (IRPC) task for the first time and propose a model named HIRPCN. 
% % 我们的方法
% By adaptively utilizing abundant semantic information and various interdisciplinary knowledge, HIRPCN can classify the multiple type text into the most fine-grain discipline or interdiscipline in the real-world dataset. \note{confusing for reviewers.
% Unlike other methods, HIRPCN can also start prediction from any given discipline label, which is practical for the online system.}
% 模型特性
Besides this, we collaborate with experts from a different domain to prove that HIRPCN can find the hidden interdisciplinary label for the research proposal, which significantly improves the whole peer-review system in government agencies. 
% 实验提一嘴
\fi
% \note{qzy:
% The development of science is indispensable to the funding supply, which needs an open-court competition organized by government agencies (e.g., NSF) for every scientist between their research proposals. 
% % 背景
% This paper study the research proposal classification problem, which is to find the most relevant discipline for research proposals to help the funding administrator allocate the proposals to suitable experts. 
% % 点出研究主题
% % 目的 - 找到最相关的学科能够协助基金管理者分配专家
% However, it is challenging to classify the research proposals into the hierarchical discipline system. Besides, due to the emergence of interdisciplinary research, the assumption of a research proposal belonging to one or two disciplines should be considered.
% %challenge
% To address that, this paper study the Interdisciplinary Research Proposal Classification (IRPC) task for the first time. We propose a model named HIRPCN. By adaptively utilizing abundant semantic information and various interdisciplinary knowledge, HIRPCN can classify the multiple type text into the most fine-grain discipline or interdiscipline in the real-world dataset.
% HIRPCN can also start from an expert given discipline to complete label prediction.
% % 模型特性
% Besides this, we collaborate with experts from a different domain to prove that HIRPCN can find the hidden interdisciplinary label for the research proposal, which significantly improves the whole peer-review system in government agencies. 
% }






==> document/dataset.tex <==
\begin{table}
\centering
\caption{The Details of Three Datasets.}
\label{dataset}
\input{document/table/dataset}
\end{table}
% \begin{table}
% \centering
% \caption{The discipline and sub-discipline numbers on each level of hierarchical discipline structure. }
% \label{disciplines}
% \input{document/table/disciplines}
% \end{table}
We collect research proposals written by the Chinese scientists from 2020's NSFC research funding application platform, containing 280683  records with 2494 ApplyID code. 7\% of the research proposal is interdiscipline research, marked by two major discipline labels. 37\%  of the research proposal contains one major discipline but shows interdisciplinarity in its subdiscipline. The rest research proposals are marked as non-interdisciplinary research by their writer. We further organized and divided the proposals by their interdisciplinarity into three datasets named \textit{RP-all}, \textit{RP-bi}, and \textit{RP-differ}. The RP-all is the overall dataset with all kinds of research proposals. The RP-bi consists of the research proposal that exhibits interdisciplinarity in the subdiscipline of their major discipline. The RP-differ only include the research proposal with two major discipline. In Table \ref{dataset}, we have counted the lengths of each label sequence and the average number of labels in each level on three different data sets. Generally speaking, from RP-all to RP-differ, its text data exhibit interdisciplinarity increasingly, and it becomes more challenging to classify correctly in the hierarchical disciplinary structure. 

% In data processing, we filter the incomplete record and group the documents in each research proposal by the type of text. We choose four parts of a research proposal as the textual data: 1) Title, 2) Keywords, 3) Abstract, 4) Research Field. The Abstract part is long-text form, and the average length is 100. The rest three documents are short text. All those documents are critical when experts judge where the proposal belongs. We further removed all the punctuation and padded the length of each text to 200. On the label side, we group the ApplyID codes by their level and add a stop token to the end of each label set sequence. 
% As shown in Table \ref{disciplines}, when the level goes deeper, since there is more number of disciplines, the classification becomes harder.

==> document/experiments_old.tex <==
In this section, we conduct experiments to evaluate the performance of HMDG from several different points of view. We first introduce the datasets, the baseline methods, the evaluation metrics, and the experiment settings. Then we compare HMDG with the baselines in Section \ref{perf com}. In the rest sections, we provided some case studies to prove the model architecture's effectiveness in HMDG. 
% The main problem we want to ask in this section is listed as follow:
% (1) Can HMDG give a accurate prediction results on three real-world proposal datasets?
% (2) Is the interdisciplinary knowledge from the Co-topic Graph can help the HMDG perform better? 
% (3) Dose HMDG have the ability to start label generation from every steps?
% (4) Are all the attention mechanisms used in HMDG interpretable and reasonable?
% (5) Can HMDG understand the dependency information on hierarchical discipline structure? 
% (6) Can HMDG give the finest-grain result for a given research proposal?
% Besides, we conduct ablation study, hyperparameter sensitivity, and model convergence experiments to explore the analyze the underlying mechanism of HMDG. 


\subsection{Baseline Methods}
To comprehensively evaluate the performances of our proposed method under the Interdisciplinary Proposal Classification task, we compare it with seven Text Classification (TC) methods including \textbf{TextCNN}\cite{textcnn},\textbf{DPCNN}\cite{dpcnn}, \textbf{FastText}\cite{fasttext1,fasttext2}, \textbf{TextRNN}\cite{textrnn}, \textbf{TextRNN-Attn}\cite{textrnnattn}, \textbf{TextRCNN}\cite{textrcnn}, \textbf{Trasnformer}\cite{vaswani2017attention} and three state-of-the-art Hierarchical Multi-label Classification (HMC) approaches including \textbf{HMCN-F}, \textbf{HMCN-R} \cite{wehrmann2018hierarchical}, \textbf{HARNN} \cite{huang2019hierarchical}. We also post two variants of HMDG as ablation baselines including \textbf{HIRPCN w/o Interdisciplinary Graph} (HIRPCN w/o IG) and \textbf{HIRPCN w/o Hierarchical Transformers} (HIRPCN w/o HT). The characteristics of these methods are listed in Table \ref{overall} with mark HA, TA, IA, and SFA. The HA represents the model's prediction process is hierarchy-aware and follows the top-down fashion. And the TA implies the model is text-type aware. The IA means that the model is equipped with Interdisciplinary Graph and is mindful of interdisciplinary knowledge. And the SFA means that due to the architecture, the model can start prediction from any given step.

\subsection{Performance Comparison}
\label{perf com}
% \usepackage{multirow}
\begin{table}
\centering
\caption{Experimental results on all dataset. The best results are highlighted in \textbf{bold}. The second-best results are highlighted in \underline{underline}}
\label{overall}
\input{document/table/overall_withnotation}
\end{table}

% \subsubsection{Performance Comparison} 
We first evaluate all methods on all datasets in Table~\ref{overall}. In this comparison, we organized every level-wise prediction result flatly, then we used \textit{Micro-F1} and \textit{Macro-F1} as the evaluation metrics, which is widely used in HMC problem~\cite{metric1, metric2, huang2019hierarchical,xiao2021expert}. From the results, we can observe that:

(1) Our proposed method, HIRPCN achieves the best performance on all datasets in all evaluation metrics, proving that HIRPCN can better solve the challenges mentioned in the IRPC task.

(2) HIRPCN w/o IG achieves equivalent performance in RP-all and RP-bi but falls back a lot on RP-differ, proving that IG and IKE can help the model in interdisciplinary prediction.

(3) HIRPCN w/o HT achieves equivalent performance to TC methods and is significantly behind HIRPCN, proving that using a hierarchical transformer structure in multi-type long-text modeling is critical.

\subsection{Case Study}
\subsubsection{Attention Mechanism Explain} We introduce the attention mechanism in most parts of HIRPCN. In this section, we visualize the word-level attention in HIRPCN for discussion. Figure~\ref{Fig.attn_text} is a case study of an interdisciplinary research proposal. As we mentioned in Section~\ref{SIE}, each representation of the word token will be aggregated by different attention values. If a word token gains more SIE's attention, they will be shading redder in this figure. From the figure, we can observe some interesting phenomena:

(1) As we hope, in the SIE, the model will pay more attention to the tokens which is more relevent to the corresponded disciplines. For example, in the \textit{Title}, the word \textit{Lung Cancer} will gain more attention due to its relation to the \textit{Life Sciences}. 

(2) Also, the attention value will be high for the word token, which is relevant to the other interdiscipline. Like the word \textit{Deep Mining Algorithm}, it has no relation to the \textit{Life Sciences}. Still, it will gain more attention by its connection to the \textit{Information Sciences}, the interdiscipline of this proposal. 

(3) Due to the self-attention mechanism, the representation of the word token won't lose semantic information in any position. Take the long-text data \textit{Abstract} as an example, the word token \textit{Mining}, \textit{Algorithm} from the \textit{Information Science} and the word token \textit{Genetic Variation} from \textit{Life Sciences} will both gain attention from the model by its relevance to the related discipline.

% \textbf{Document-level Attention}: As described before, HIRPCN follows a top-down fashion in discipline path generation. In each step of prediction, we hope the model can pay adaptive attention to the different parts of the proposal.

\begin{figure}
\centering
\includegraphics[width=0.50\textwidth]{figure/HIRPCN-case-proposal_attention.eps} 
\caption{A interdisciplinary research proposal and its word-level attention visualization from the \textit{Information Sciences} and the \textit{Life Sciences}}
\label{Fig.attn_text}
\end{figure}
% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{figure/attention_previous.eps} 
% \caption{}
% \label{Fig.attn_pre}
% \end{figure}
% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{figure/attention_text_type.eps} 
% \caption{}
% \label{Fig.attn_type}
% \end{figure}

\subsubsection{Expert Evaluation}
During the performance experiment on dataset RP-all, we find that model will predict an additional discipline for some research proposals along their truth label. 
\begin{figure}
\centering
\includegraphics[width=0.45\textwidth]{figure/evalresult.pdf} 
\caption{}
\label{Fig.evalresult}
\end{figure}

We illustrate four research proposals where the HIRPCN finds it is related to \textit{Information Sciences}.

\begin{figure}
\centering
\includegraphics[width=0.50\textwidth]{figure/wrongcasestudy.eps} 
\caption{}
\label{Fig.wrong_case}
\end{figure}

\subsubsection{Start Prediction From Anywhere Evaluation}
Due to the design of the architecture, the HIRPCN can start prediction from any give partial label and generate the rest. We further test the performance when the partial label from different level is given. As you can see in the Figure~\ref{Fig.partial_label}, 
\begin{figure}
\centering
\includegraphics[width=0.45\textwidth]{figure/partial_label.pdf} 
\caption{}
\label{Fig.partial_label}
\end{figure}
\subsubsection{Granular of Prediction}

\begin{table}
\centering
\caption{Experimental results on RP-differ in level-wise. The best results are highlighted in \textbf{bold}. The second-best results are highlighted in \underline{underline}}
\label{RPdiffer}
\input{document/table/differ-f1}
\end{table}

==> document/method_before_sim.tex <==
\section{Interdisciplinary Label Path Detection}

\begin{figure}[t!h]
\centering
\includegraphics[width=0.50\textwidth]{figure/model_overall_word.pdf} 
\caption{An overview figure of the HIRPCN during the $(k)$-th step prediction.}
\label{Fig.model_1}
\end{figure}

\subsection{Overview of the Proposed Framework} Figure~\ref{Fig.model_1} show our  framework iterate four steps: 
1) Semantic Information Extractor (SIE), 2) Interdisciplinary Knowledge Extractor (IKE), 3) Information Fusion (IF), and 4) the Level-wise Prediction (LP).
The SIE models the type-specific semantic information (e.g., title, abstract, keywords, research fields) in research proposals.
The IKE learns discipline label embedding at current depth by modeling both  interdisciplinary graph and predicted topics labels of shorter depth
The IF fuses the representations of each document in a proposal and topic label embedding.
The LP predicts each discipline's probability to identify the discipline label at current depth of the three. 
After the completion of the iteration, our framework take predicted discipline labels at current depth and start to predict fine-grained discipline next depth. 


\begin{figure}[t!h]
\centering
\includegraphics[width=0.50\textwidth]{figure/encoder_pe_v1.pdf} 
\caption{\textit{Semantic Information Extractor}. 
The input of SIE is a set of type token and their related document. The $\bullet$ means a linear transform operation followed by an element-wise addition.}
\label{Fig.model_encoder}
\end{figure}

\subsection{Semantic Information Extractor}\label{SIE}
Figure~\ref{Fig.model_encoder} shows an overview of SIE. The basic idea is to learn the representations of the textual data of a proposal. 
A proposal includes a set of documents (e.g., title, abstract, key words, research fields), each of which includes a sequence of words.
To learn the representation of a proposal, the SIE is structured to include a word to vec layer, a Multiple Positional Encoding (MPE) layer, and a SIEBlock that consists of two building blocks:  1) a word-level Transformer~\cite{vaswani2017attention}  and 2) a document-level Transformer. Formally, the embedding of a proposal is learned by:  
\begin{equation}
    \mathbf{e}_D 
    = N_e \times SIEBlock(MPE(\mathbf{W}^{(0)})),
\end{equation}
where the matrix $\mathbf{e}_D$ is the embedding of  the textual data and document type information of  the document set of a proposal $D$. 
$\mathbf{W}^{(0)}=\{\mathbf{w}_1^{(0)}, \mathbf{w}_2^{(0)}, ..., \mathbf{w}_{|T|}^{(0)}\}$ is the initial word embedding set of each documents in $D$. $\mathbf{w}_i^{(0)} \in \mathbb{R}^{|d_i| \times h}$ is the word embedding matrix of document $d_i$. The $N_e$ is the total layer number of SIE Block. The $MPE(\cdot)$ means a positional encoding for each $\mathbf{w}_i^{(0)}\in \mathbf{W}^{(0)}$. 


\noindent\textbf{Our Perspective: Modeling Texts and Document Type for Proposal Embedding.} We consider two essential aspects of a proposal. Firstly, each document (e.g., a title's texts) in a proposal vary in terms of length, and some document is very short. A short concatenated text will cause a severe loss of long-term dependency. 
Secondly, different types (e.g., title, abstract, keywords, research fields) of documents in a research proposal have different weights in identifying the disciplines of the proposal.
Inspired by the long-text modeling methods~\cite{pappagari2019hierarchical,zhang2019hibert,liu2019hierarchical}, we design a \textit{hierarchical transformer architecture}  to model both texts and document type information of a proposal into latent neural embedding. 

\noindent\textbf{Step 1: Word2Vec and Multilple Positional Encoding.} 
% The first input matrix $\mathbf{w}^{(0)}_{i}$ of document $d_i$ is the word embeddings corresponding with $[w^{i}_1,w^{i}_2,...,w^{i}_{|d_i|}]$, 
We convert words of each document in a proposal into initial embedding (denoted by the matrix $\mathbf{w}^{(0)}_{i}$ of document $d_i$) by pre-trained $h$-dimensional Word2Vec~\cite{mikolov2013distributed} model and sum with positional encoding to preserve the position information.

\noindent\textbf{Step 2: Word-level Transformer}
In the first stage of SIEBlock, for each document $d_i$, we aim to use a Word-level Transformer to extract the contextual semantic information of the document representation matrix $\mathbf{w}^{(l-1)}_{i}$ of $d_i$ from previous layer to obtain $\mathbf{w}^{(l)}_{i}$, fomulated as:
\begin{equation}
\begin{aligned}
    \mathbf{w}^{(l)}_{i} &= Transformer_{w}(\mathbf{w}^{(l-1)}_i),
\end{aligned}
\end{equation}
where $l$ is the current layer number of SIEBlock, the $\mathbf{w}^{(l)}_i \in \mathbb{R}^{|d_i| \times h}$ is the vanilla document representation matrix and each row is a word embedding. 

\noindent\textbf{Step 3: Document-level Transformer:}
In each layer of the Document-level Transformer, we  integrate the type information with the vanilla document representation matrix and feed each document's type-specific representation into the Transformer. To incorporate the type information, inspired by ViT\cite{dosovitskiy2020image} and TNT\cite{han2021transformer}, we first use a fully-connected layer to transform the vectorized vanilla document representation to a vector. Next, the vector will element-wisely  add with its type-token vector to get the type-specific representation. The current layer's type-specific representation $\hat{e}^{(l-1)}_{d_i}$ of document $d_i$ is obtained by:
\begin{equation}
\label{ew2}
    \begin{aligned}
    \hat{e}^{(l-1)}_{d_i}=e^{(l-1)}_{d_i} + FC(Vec(\mathbf{w}^{(l)}_{i})),
\end{aligned}
\end{equation}
After obtain the  $\hat{\mathbf{e}}^{(l-1)}_D=\{\hat{e}^{(l-1)}_{d_1}, \hat{e}^{(l-1)}_{d_2}, ... ,\hat{e}^{(l-1)}_{d_{|T|}}\}$, we \textbf{\color{red} put the type-specific documents' representations set} to the document-level Transformer in layer-$l$: 
\begin{equation}
\begin{aligned}
    \label{trans2}
    \mathbf{e}^{(l)}_{D} = {Transformer}_{d}(\hat{\mathbf{e}}^{(l-1)}_D), 
\end{aligned}
\end{equation}
where ${Transformer}_{d}(\cdot)$ is a Document-level Transformer, $\mathbf{e}^{(l)}_{D}\in \mathbb{R}^{|T| \times h}$ is the outputs, which can be seen as $|T|$-views of high-level abstraction for proposals.


% To incorporate the type information, inspired by ViT\cite{dosovitskiy2020image} and TNT\cite{han2021transformer}, we first use a fully-connected layer to transform the vectorized vanilla document representation to a vector. Next, the vector will element-wise add with its \textbf{type-token} vector to get the type-specific representation. The current layer's type-specific representation $\hat{e}^{(l-1)}_{d_i}$ of document $d_i$ is obtained by:

% where $e^{(l-1)}_{d_i} \in \mathbb{R}^h$ is the representation of document $d_i$ from previous layer of document-level Transformer. The input vector $e^{(0)}_{d_i}$ in first layer is a random initialized vector for type token $t_i$. The $FC(\cdot)$ is a fully-connected layer, and the $Vec(\cdot)$ is the vectorization operation. The $\hat{e}^{(l-1)}_{d_i} \in \mathbb{R}^h$ is the type-specific representation of the document $d_i$ in current layer $l$. 

% After obtain the  $\hat{\mathbf{e}}^{(l-1)}_D=\{\hat{e}^{(l-1)}_{d_1}, \hat{e}^{(l-1)}_{d_2}, ... ,\hat{e}^{(l-1)}_{d_{|T|}}\}$ from the Word-level Transformer, we put the type-specific documents' representations set to the document-level Transformer in layer-$l$: 
% \begin{equation}
% \begin{aligned}
%     \mathbf{e}^{(l)}_{D} & = \{e^{(l)}_{d_1}, e^{(l)}_{d_2}, ..., 
%     e^{(l)}_{d_{|T|}}\} \\
%     &= {Transformer}_{d}(\hat{\mathbf{e}}^{(l-1)}_D), 
% \end{aligned}
% \end{equation}
% where ${Transformer}_{d}(\cdot)$ is a Transformer to extract the document-level features for proposals, $\mathbf{e}^{(l)}_{D}\in \mathbb{R}^{|T| \times h}$ is the Transformer outputs, which can be reviewed as $T$-views of high-level abstraction for proposals. 



\begin{figure}[!th]
\centering
\includegraphics[width=0.45\textwidth]{figure/encoder_2.eps} 
\caption{The \textit{Interdisciplinary Knowledge Extractor}. The different colors of the node in $\mathbb{L}_{<k}$ and sub-graph represent different disciplines. The red outline marks each central node.}
\label{Fig.model_encoder_2}
\end{figure}

\subsection{Interdisciplinary Knowledge Extractor}
% \note{As we aim to infer the Interdisciplinary label, the relations between disciplinary need to be incorporated. The disciplinary tree only contains single disciplinary information, thus, we introduce the co-word graph.}

After learning the proposal embedding, we need to learn discipline label embeddings to iteratively predict discipline label path for a proposal.  
Figure \ref{Fig.model_encoder_2} shows a multi-layer Graph Convolution Networks. We construct an interdisciplinary label-label graph and then leverage the predicted discipline labels and the interdisciplinary label-label graph  

Our idea is the model will pass a subgraph of the predicted label on the Interdisciplinary Graph between each step rather than the label itself, which helps to provide the \textbf{interdisciplinary knowledge} for the label prediction in the next level.
% We design this structure for two reasons: 1) the subgraph will increase each label's receptive field and provide the topological structure of \textbf{interdisciplinary cooperation knowledge}.
% \note{qzy: why it is a reason?
% 2) we can initialize the prediction from any given \textbf{partial label} by the IKE module.}

Given the sequence of label sets $\mathbb{L}_{<k}$ generated from previous $k-1$ steps prediction (or from a given partial label from expert) as input, where $\mathbb{L}_{<k} = [L_{0}, L_1,..., L_{k-1}]$. 
Each label set $L_i=\{l_i^j\}_{j=1}^{|L_i|}$ holds the prediction result in the $i$-th level and consist of the discipline labels. 
% We aim to learn the interdisciplinary knowledge of each $L_i$ with other related disciplines on the Interdisciplinary Graph $\mathcal{G}$. 
We first treat each discipline label in every set as a central node and sample its $N_g$-hops sub-graph from $\mathcal{G}$, where the $N_g$ is the layer number of GCNs. Then we pass the sub-graph set $\hat{\mathcal{G}}_{<k}=\{\hat{\mathcal{G}}_0, \hat{\mathcal{G}}_1,...,\hat{\mathcal{G}}_{k-1}\}$ and their node features into $N_g$ layers of GCNs and a \textit{Readout} layer to obtain $e_{L_i}$:
\begin{equation}
\begin{aligned}
    \mathcal{H}^{(N_g)}_i &= N_g \times GCNLayer(\hat{\mathcal{W}}_i, \hat{\mathcal{H}}^{(0)}_i),\\
    e_{L_i}& = Readout(\mathcal{H}^{(N_g)}_i, L_i),
\end{aligned}
\end{equation}
where the $\hat{\mathcal{H}}^{(0)}_i$ is the random initialized features of each node in sub-graph $\hat{\mathcal{G}}_i$ and the $\hat{\mathcal{W}}_i$ is the weighted adjacency matrix of $\hat{\mathcal{G}}_i$. The $\mathcal{H}^{(N_g)}_i$ is a hidden output matrix undergoing $N_g$ times GCN layers propagate on the sub-graph. The \textit{Readout} layer is to get the representations of the central nodes from $\mathcal{H}^{(N_g)}_i$, which can be a lookup operation, a mean pooling operation, or a self-attention layer
% ~\cite{lee2019self}
, etc. For simplicity, we set the readout as a lookup operation to achieve the index of nodes in $L_i$ on $\mathcal{H}^{(N_g)}_i$.
% \note{? after a lookup operation via the index of nodes in $L_i$ on $\mathcal{H}^{(N_g)}_i$}. 
The $e_{L_i} \in \mathbb{R}^h$ is the final representation of $i$-th label set $L_i$. Then we can form the representation of sequence of label set $\mathbb{L}_{<k}$ as $\mathbf{e}_{\tiny \mathbb{L}_{<k}}=[e_{\tiny L_0}, e_{\tiny L_1},...,e_{\tiny L_{k-1}}]$. The $\mathbf{e}_{\tiny \mathbb{L}_{<k}}$ can be seen as the representation of the prediction result from the previous $k-1$ step integrated with interdisciplinary knowledge.
\begin{figure}
\centering
\includegraphics[width=0.45\textwidth]{figure/Decoder.pdf} 
\caption{\textit{Information Fusion} and \textit{Level-wise Prediction} in step-$k$. }
% The left side of this figure illustrate the structure of Information Fusion component. The input is the information from previous $k-1$ step prediction and the semantic information of research proposal extracted from SIE. After $N_d$ times iteration of IF Block process, we can obtain the fusion matrix $\mathbf{S}_k$. The right side is the Level-wise prediction component, which will utilize the hierarchical information from hierarchical discipline structure $\gamma$ and the fusion matrix $\mathbf{S}_k$ to generate step-$k$ prediction results.
\label{Fig.model_decoder}
\end{figure}
\subsection{Information Fusion}
% The IF aims to integrate the semantic information and previous prediction results with disciplinary knowledge via the \textit{Multi-Head Self-Attention Mechanism}. 
The IF component follows a multi-layer design, and each layer is named \textit{IF Block}. As you can see in the left side of Figure \ref{Fig.model_decoder}, in each layer, the first step of IF aims to integrate the previous prediction results with disciplinary knowledge from IKE via the \textit{Multi-Head Self-Attention}. And the rest is designed to aggregate the semantic information according to the integrated prediction result. 

Formally, from the IKE, we can obtain the representation of former prediction result with interdisciplinary knowledge $\mathbf{e}_{\tiny \mathbb{L}_{<k}}$. We start with sum the embedding with corresponding positional encoding as the input $\mathbf{S}^{(0)}_{\tiny <k}=\{s^{(0)}_{root},s^{(0)}_{1},s^{(0)}_{2},...,s^{(0)}_{k-1}\}$:
\begin{equation}
\begin{aligned}
    \label{pe}
    \mathbf{S}_{<k}^{(0)}=PE(\mathbf{e}_{\tiny \mathbb{L}_{<k}}),
\end{aligned}
\end{equation}
where $PE(\cdot)$ is the positional encoding function.

After that, in each layer of IFBlock, we perform multi-head attention-based propagation with a \textit{Residual Connection and Normalization Layer} between each prediction result representation to help $s_i^{(l)} \in \mathbf{S}_{<k}^{(l)}$ learn dependency information from their context: 
\begin{equation}
\label{M}
    \hat{\mathbf{S}}_{<k}^{(l-1)} = \sigma( \mathbf{S}_{<k}^{(l-1)}+ MultiHead(\mathbf{S}_{<k}^{(l-1)},\mathbf{S}_{<k}^{(l-1)},\mathbf{S}_{<k}^{(l-1)})),
\end{equation}
where the $\hat{\mathbf{S}}_{<k}^{(l)} \in \mathbb{R}^{k\times h}$ preserves the ancestor labels information.

Then, we feed the output $\hat{\mathbf{S}}_{<k}^{(l-1)}$ and proposal representation $\mathbf{e}_D$ into a \textit{Multi-head Attention Layer}, a \textit{Residual Connection and Normalization Layer}, a \textit{Feed Forward Layer}, and a \textit{Residual Connection and Normalization Layer} to propagate the semantic information depending on the previous prediction result: 
\begin{equation}
\label{Z}
    Z^{(l-1)} = \sigma(\hat{\mathbf{S}}_{<k}^{(l-1)} + MultiHead(\hat{\mathbf{S}}_{<k}^{(l-1)} , \mathbf{e}_D, \mathbf{e}_D)),
\end{equation}
\begin{equation}
\label{L}
    \mathbf{S}_{<k}^{(l)} =  \sigma(Z^{(l-1)}+\mathcal{F}(Z^{(l-1)})),
\end{equation}
where $\hat{\mathbf{S}}_{<k}^{(l)}$ is the query, $\mathbf{e}_D$ is the key and value, which aims to extract information from the proposal corresponding to the predicted labels. The output of this layer is the hidden embeddings $\mathbf{S}_{<k}^{(l)} =[s^{(l)}_{root},s^{(l)}_{1},s^{(l)}_{2},...,s^{(l)}_{k-1}]$, where each $s^{(l)}_i$ can be seen as a representation of the proposal which is correlated with the label $l_i$. 

Finally, we stack $N_d$ layers of the above components and obtain the final output in the last layer:
% = \mathbf{S}_{<k}^{(N_d)}
% \begin{equation}
% \begin{aligned}
%     \mathbf{S}_{k} &  = [s^{\tiny(N_d)}_{root},s^{\tiny (N_d)}_1,s^{\tiny (N_d)}_2,...,s^{\tiny (N_d)}_{k-1}] \\
%     &=N_d \times IFBlock(\mathbf{e}_{\tiny \mathbb{L}_{<k}}, \mathbf{e}_D),
% \end{aligned}
% \end{equation}
\begin{equation}
\begin{aligned}
    \mathbf{S}_{k} =N_d \times IFBlock(\mathbf{e}_{\tiny \mathbb{L}_{<k}}, \mathbf{e}_D),
\end{aligned}
\end{equation}
where $N_d$ is the total layer number of IF Block, and $\mathbf{S}_{k}\in \mathbb{R}^{k\times h}$ is the fusion matrix that integrated the proposal information with $k$ previous ancestor labels of the proposal.
\iffalse
After that, given $\mathbf{S}^{(l-1)}_{\tiny <k}$ and semantic information $\mathbf{e}_D$, the propagation of the $l$-th layer in the IF is defined as:\note{specific, resual, feed forword, etc}
\begin{equation}
\label{M}
    \hat{\mathbf{S}}_{<k}^{(l-1)} = \sigma( \mathbf{S}_{<k}^{(l-1)}+ MultiHead(\mathbf{S}_{<k}^{(l-1)},\mathbf{S}_{<k}^{(l-1)},\mathbf{S}_{<k}^{(l-1)})),
\end{equation}

% The second stage of IF is a source attention component:

\begin{equation}
\label{Z}
    Z^{(l-1)} = \sigma(\hat{\mathbf{S}}_{<k}^{(l-1)} + MultiHead(\hat{\mathbf{S}}_{<k}^{(l-1)} , \mathbf{e}_D, \mathbf{e}_D)),
\end{equation}

\begin{equation}
\label{L}
    \mathbf{S}_{<k}^{(l)} =  \sigma(Z^{(l-1)}+\mathcal{F}(Z^{(l-1)})),
\end{equation}
where the propagation can be divided into two stages. In Equation \ref{M}, the input label is feeded into a multi-head self-attention layer to capture the dependency between labels in the label set, and the output $\hat{\mathbf{S}}_{<k}^{(l)} \in \mathbb{R}^{k\times h}$ preserves the ancestor labels information. In Equation \ref{Z} and \ref{L}, $\hat{\mathbf{S}}_{<k}^{(l)}$ is incorporated with the proposal representation matrix $\mathbf{e}_D$ via a source attention layer, where $\hat{\mathbf{S}}_{<k}^{(l)}$ is the query, $\mathbf{e}_D$ is the key and value, which aims to extract information from the proposal corresponding to the predicted labels. The output of this layer is the hidden embeddings $\mathbf{S}_{<k}^{(l)} =[s^{(l)}_{root},s^{(l)}_{1},s^{(l)}_{2},...,s^{(l)}_{k-1}]$, where each $s^{(l)}_i$ can be seen as a representation of the proposal which is correlated with the label $l_i$. 
Finally, We stack $N_d$ layers of the above components and obtain the final output in the last layer:
% = \mathbf{S}_{<k}^{(N_d)}
\begin{equation}
\begin{aligned}
    \mathbf{S}_{k} &  = [s^{\tiny(N_d)}_{root},s^{\tiny (N_d)}_1,s^{\tiny (N_d)}_2,...,s^{\tiny (N_d)}_{k-1}] \\
    &=N_d \times IFBlock(\mathbf{e}_{\tiny \mathbb{L}_{<k}}, \mathbf{e}_D)
\end{aligned}
\end{equation}
where $\mathbf{S}_{k}\in \mathbb{R}^{k\times h}$ is the fusion feature matrix that integrated the proposal information with $k$ previous ancestor labels of the proposal, And $N_d$ is the total layer number of IF Block.
\fi
\subsection{Level-wise Prediction}
% According to Equation \ref{equation_1}, we hope that the HIRPCN can generate labels set in a \textbf{top-down fashion} from the beginning level to a \textbf{proper} level $H_A$. 
The right side of Figure \ref{Fig.model_decoder} demonstrate the prediction in step-$k$. In LP, We feed the fusion feature matrix $\mathbf{S}_{k}$ into a pooling function, a fully connected layer, and a Sigmoid layer to generate each label's probability for $k$-th level-wise label prediction. In our paper, we set this pooling function as directly taking the last vector of $\mathbf{S}_{k}$. The formal definition is:
\begin{equation}
 {\hat{y}}_k= Sigmoid({\mathcal{F}}_{k}(Pooling(\mathbf{S}_{k}))),
\end{equation}
where $\hat{y}^i_k\in [0,1]$ is the predicted probability of the $i$-th discipline $c^i_k$ in level-$k$ $c^i_k \in C_k$. The $\mathcal{F}_{k}(\cdot)$ denotes a level-specific feed-forward network with ReLU activation function to project the input to a $|C_k|+1$ length vector. 
After the $Sigmoid(\cdot)$, the final output $\hat{y}_k$ is the probability of $k$-th level's labels. 
In prediction progress, the label corresponding to the index of the value in the $\hat{y}_k$ that achieves the threshold will be selected to construct the current prediction result.

We require that the model can define a distribution over labels of all possible lengths, we add a \textbf{end-of-prediction label} $l_{stop}$ token and set the first element of $\hat{y}_k$ as the probability of $l_{stop}$ in level-k. In the final step, the $l_{stop}$ is the prediction result, and the prediction process should end in the level-($H_A$). 
Thus, the level-$k$'s objective function $\mathcal{L}_k$ can be defined as:

% \begin{equation}
% \begin{aligned}
%     \mathcal{L}_k(\Theta)    &= \log(P(L_k|D,\gamma,\mathcal{G},\mathbb{L}_{<k}; \Theta))\\
%      &= \sum^{|C_k| + 1}_{i=1} \left(y_i \log(\hat{y}_k^i) + (1 - y_i) \log(1 - \hat{y}_k^i) \right), \\
% \end{aligned}
% \end{equation}
\begin{equation}
    \mathcal{L}_k(\Theta) = \sum^{|C_k| + 1}_{i=1} \left(y_i \log(\hat{y}_k^i) + (1 - y_i) \log(1 - \hat{y}_k^i) \right),
\end{equation} 
where $y_i=\mathbbm{1}(l_i \in L_k)$, which aims to discriminate whether the $i$-th label $l_i$ belongs to the truth label set or not. 
% Finally, after the prediction from level-$1$ to level-$H_A$, the overall objective function for each proposal $A$ with document set $D$ is to maximize the log-likelihood of the overall probability:
% % \begin{equation}
% %         \Theta = \mathop{\arg\max}_{\Theta}\sum_{k=1}^{H_A} \log P(L_k|D,\gamma,\mathcal{G},\mathbb{L}_{<k}; \Theta)
% % \end{equation}
% \begin{equation}
% \begin{aligned}
%     \mathcal{L}_k(\Theta)    &= \log(P(L_k|D,\gamma,\mathcal{G},\mathbb{L}_{<k}; \Theta))\\
%      &= \sum^{|C_k| + 1}_{i=1} \left(y_i \log(\hat{y}_k^i) + (1 - y_i) \log(1 - \hat{y}_k^i) \right) \\
% \end{aligned}
% \end{equation}
% where the $L_k$ is the ground truth label set of level-$k$ prediction. And $y_i=\mathbbm{1}(l_i \in L_k)$, which aims to discriminate whether the $i$-th label $l_i$ belongs to the truth label set or not.  

==> document/method_old.tex <==
\begin{figure}
\centering
\includegraphics[width=0.48\textwidth]{figure/model_overall_light.eps} 
\caption{An overview figure of the HMDG. In this figure, we illustrate the $k$-th step and the last step of the prediction. The $+$ operation means concatenate a set into a sequence of sets. In each step, HMDG will generate the current label set and concatenate it to the previous label set sequence.}
\label{Fig.model_1}
\end{figure}
In this section, we introduce the proposed model named HIRPCN for the IRPC task. 
The HIRPCN is divided into three parts: \textit{Information Extractor}, \textit{Information Fusion}, \textit{Level-wise Prediction}.
The Semantic Information Extractor encode the document set $D$ into vectorized representations. The Interdisciplinary Knowledge Extractor integrate the previous prediction results with the structural information from $\mathcal{G}$ into the label embedding.
In each prediction step, the Information Fusion combines the documents' representations and the label embedding from the previous steps. And the Level-wise Prediction component computes the conditional probability of each label on the current level.

\iffalse
In this section, we detailedly introduce our model named \textbf{H}ierarchical \textbf{M}ulti-\textbf{d}iscipline \textbf{G}enerator (HMDG) and explain how we extract the information from the research proposal properly to preserve the multiple type characteristic in each text. And how we explore the information from Hierarchical Discipline Structure and Interdisciplinary Graph to guild the process of length-variable label set sequence generation with type-specific semantic information via a top-down fashion. 
From the purpose of each step, we can divide the HMDG into three parts: \textit{Information Extractor}, \textit{Information Fusion}, \textit{Level-wise Prediction}. We overview the model in Section 3.1, and we give a detailed demonstration of those parts in the rest sections.
\fi


\iffalse
In our model, the set of documents $D$ in a proposal $A$ and the Interdisciplinary Graph $\mathcal{G}$ serves as the input. The generated output is a sequence of label sets $\mathbb{L} = [L_1, L_2,..., L_{H_A}]$ with length $H_A$, which describes several paths from the root to the most fine-grained discipline on the hierarchical discipline structure $\gamma$.
\fi

\iffalse
\subsection{Model Overview}
The HMDG is divided into three parts: \textit{Information Extractor}, \textit{Information Fusion}, \textit{Level-wise Prediction}.
As shown in Figure \ref{Fig.model_1}, we decompose the prediction process into an up-to-down fashion from the beginning level to a certain level on the hierarchical discipline structure $\gamma$.
The Semantic Information Extractor first encode the document set $D$ into vectorized representations. Then, the Interdisciplinary Knowledge Extractor integrate the previous prediction results with the structural information from $\mathcal{G}$ into the label embedding.
In each prediction step, the Information Fusion combines the documents' representations and the label embedding from the previous steps. And the Level-wise Prediction component computes the conditional probability of each label on the current level.
%For the first level, we add $L_{0}=\{l_{root}\}$, which contains the root node of $\gamma$, to the initial sequence $\mathbb{L}_{<1}$, as the input label set sequence. Also, to define the probability over the length $H_A$, we add a particular end-of-prediction token $l_{stop}$, which enables the iterative process of the model to stop on the proper step when the label $l_{stop}$ is predicted. 
Suppose the $k-1$ ancestors labels in $L$ is $\mathbb{L}_{<k} = [L_{0}, L_1,..., L_{k-1}]$, where $\mathbb{L}_{<1}=\{L_0\}$,
the prediction on level $k$ can be formed as:
$$\Omega(D,\mathbb{L}_{<k},\gamma,\mathcal{G},\Theta) \to L_{k}$$

Eventually, we can formulate the probability of the assignment of the sequence of label sets for the proposal as:
\begin{equation}
    P(\mathbb{L}|D,\gamma,\mathcal{G};\Theta)=\prod_{k=1}^{H_A+1} P(L_k|D,\gamma,\mathcal{G},\mathbb{L}_{<k}; \Theta)
    \label{equation_1}
\end{equation}

where $ P(\mathbb{L}|D,\gamma,\mathcal{G};\Theta)$ is the overall probability of the proposal $A$ belonging to the label set sequence $\mathbb{L}$, $P(L_k|D,\gamma,\mathcal{G},\mathbb{L}_{<k}; \Theta)$ is the label set assignment probability of $A$ in level $k$ when given the previous ancestor $\mathbb{L}_{<k}$.
In training, given all the ground truth labels, our goal is to maximize the Equation \ref{equation_1}.
% In this way, our model can be regarded as an encoder-decoder framework. Similar to the translation model, the encoder extracts textual information from the documents, and the decoder generates the labels of proposals on the hierarchical discipline structure.

\fi

\subsection{Information Extractor}
In this section, we introduce the encoder of the HIRPCN named \textit{Information Extractor} (IE), which is composed of two components. The first component, named \textit{Semantic Information Extractor} (SIE), aims to capture the rich semantic information from the input research proposal's document set $D$. Besides, we design the second component named \textit{Interdisciplinary Knowledge Extractor} (IKE) to capture the interdisciplinary information from the Interdisciplinary Graph.
%The first component, named \textit{Semantic Information Extractor} (SIE), aims to capture the semantic information from the input research proposal's document set $D$ and to extract the relationship between each type of documents by hierarchical Transformer structure. Besides, we design the second component named \textit{Interdisciplinary Knowledge Extractor} (IKE) to initial the domain knowledge for each discipline label. 
% \note{qzy:  The first component, named \textit{Semantic Information Extractor} (SIE), aims to capture the rich semantic information from the input research proposal's document set $D$ via a hierarchical Transformer extractor. Besides, we design the second component named \textit{Interdisciplinary Knowledge Extractor} (IKE) to capture the cross interdisciplinary information and initialize the representation of each discipline label.}


\begin{figure}
\centering
\includegraphics[width=0.48\textwidth]{figure/SIE.eps} 
\caption{\textit{Semantic Information Extractor}. The input of SIE is a set of type token and their related document. The $\bullet$ means a linear transform operation followed by an element-wise addition.}
\label{Fig.model_encoder}
\end{figure}


\subsubsection{Semantic Information Extractor}\label{SIE}
% \note{type token is critical to this component, but in general, i cannot find the footprint of it. To overcome this, try to modify the illustration on Research Proposal and the SIE in this layer}
\iffalse
To extract the semantic information in a given Proposal $A$, a simple solution is to concatenate all its words into a flat text sequence as the input. 
% (e.g., the Flat Encoder in Figure\ref{Fig.model_encoder}(1)). 
However, on the one hand, the input sequence would be extremely long, which would be computationally intensive for the encoding of the Transformer according to Equation \ref{eq5}-\ref{eq7}. 
On the other hand, the simple concatenation ignores the uniqueness between different text types, undermining the model's effectiveness. 
Recently, hierarchical Transformer structure is widely adopt in modeling neural language and long-text documents \cite{pappagari2019hierarchical,zhang2019hibert,liu2019hierarchical}.
Thus, we propose a hierarchical textual encoder for proposal feature extracting named \textit{Semantic Information Extractor}. 
% Figure \ref{Fig.model_encoder}(2-4) shows the three different structures of the SIE. 
\fi
An overview of the SIE architecture is present in Figure \ref{Fig.model_encoder}, which illustrates a multi-layer structure. Each layer of SIE is called \textit{SIE Block} which consists of a word-level Transformer and a document-level Transformer (The detail of Transformer is listed in Appedix \ref{}).\note{appedix} 
The raw documents $D$ in proposal data $A$ is first split into multiple documents $D = \{d_1, d_2,...,d_{|T|}\}$ in terms of document types. 
%Each document is followed by a type token to mark its unique type information. 
A specific type token is added in front of each document to mark its unique type information.
First, a linear embedding layer is applied on the raw document and its type token to project it to an arbitrary dimension (denoted as $h$). To note that the embedding layer of word token and type token is initialized by a pre-trained $h$-dimensional word embedding model (e.g., Word2Vec\cite{mikolov2013distributed} model) and a random embedding layer, respectively.
Then, in each SIE Block, we use the word-level Transformer separately to get the vanilla document representations. After that, the Document-level Transformer is proposed to extract the document features with the type-token and generate the representation matrix of the input documents set. 
With multiple layers of SIE Block (the total number of layers is denoted as $N_e$), we obtain the final output as $\mathbf{e}_D$ to represent the proposal both with type information and semantic information. 
Specifically, the detailed definition of the $l$-th layer of SIE block is described as follow:

\textbf{Word-level Transformer:}
In the first stage of SIE Block, for each document $d_i$, we aim to use a word-level Transformer to extract the contextual semantic information of the document representation matrix $\mathbf{w}^{(l-1)}_{i}$ of $d_i$ from previous layer to obtain $\mathbf{w}^{(l)}_{i}$, fomulated as:

\begin{equation}
\begin{aligned}
    \mathbf{w}^{(l)}_{i} &= Transformer_{w}(\mathbf{w}^{(l-1)}_i),
\end{aligned}
\end{equation}

where $l$ is the current layer number of SIE Block, the $\mathbf{w}^{(l)}_i \in \mathbb{R}^{|d_i| \times h}$ is the vanilla document representation matrix and each row is a word embedding, and the first input matrix $\mathbf{w}^{(0)}_{i}$ of document $d_i$ is the word embeddings corresponding with $[w^{i}_1,w^{i}_2,...,w^{i}_{|d_i|}]$, initialized by pre-trained $h$-dimensional Word2Vec model.

\iffalse
In the first stage of SIE Block, we aim to use a word-level Transformer to embed the input embedding $\mathbf{W}^{(l-1)}_{i}$ from previous layer into the vanilla document representation matrix $\mathbf{W}^{(l)}_{i}$, where $l$ is the current layer number of SIE Block and the $\mathbf{W}^{(l)}_i \in \mathbb{R}^{|d_i| \times h}$ is a matrix represent the vanilla feature of a document $d_i$ from word-level Transformer in layer $l$. As we mention before, the first input matrix $\mathbf{W}^{(0)}_{i}$ of document $d_i$ is initialized by  pre-trained $h$-dimensional Word2Vec model.
Then we adopt the Transformer to obtain its representation matrix for document $d_i$ in each layer:
\begin{equation}
\begin{aligned}
    \mathbf{W}^{(l)}_{i} &= Transformer_{w}(\mathbf{W}^{(l-1)}_i),
\end{aligned}
\end{equation}
where $Transformer_{w}(\cdot)$ is a Transformer to extract the word-level text feature. 
% For each token ${w}^{i}_j \in d_i$, its input vector is constructed by summing its embedding with its corresponding positional embedding in documents. 
\fi

\iffalse
In the document-level Transformer, we first use the type information of document to obtain the type-specific representation by the Multi-head Attention Layer in Equation \ref{eq5}. To note that in every first layer of SIE Block, each type token is represented by a random initialized vector. The current layer's type-specific representation $\hat{e}^{(l-1)}_{d_i}$ of document $d_i$ is obtained by:
\fi

To incorporate the type information, inspired by ViT\cite{dosovitskiy2020image} and TNT\cite{han2021transformer}, we first use a fully-connected layer to transform the dimension of  the vanilla document representation matrix $\mathbf{w}^{(l)}_{i}$. Then, we element-wise add the vector with its type token vector. The current layer's type-specific representation $\hat{e}^{(l-1)}_{d_i}$ of document $d_i$ is obtained by:
\iffalse
\begin{equation}
\label{ew2}
\begin{aligned}
\hat{e}^{(l-1)}_{d_i}=e^{(l-1)}_{d_i} + Sum(MultiHead(e^{(l-1)}_{d_i}, \mathbf{w}_{i}, \mathbf{w}_{i})),
\end{aligned}
\end{equation}
\fi
\begin{equation}
\label{ew2}
\begin{aligned}
\hat{e}^{(l-1)}_{d_i}=e^{(l-1)}_{d_i} + FC(\mathbf{W}^{(l)}_{i}),
\end{aligned}
\end{equation}
where $e^{(l-1)}_{d_i} \in \mathbb{R}^h$ is the representation of document $d_i$ from previous layer of document-level Transformer. The input vector $e^{(0)}_{d_i}$ is a random initialized vector for type token $t_i$. The $FC(\cdot)$ is a fully-connected layer. And the $\hat{e}^{(l-1)}_{d_i} \in \mathbb{R}^h$ is the type-specific representation of the document $d_i$ in current layer $l$. 

% There are two reasons for us to design the word-level transformer:\note{need revise}
% % 有多种方法采用了type-token来整合信息
% 1) There are many approaches to integrate the class information within the Transformer structure (e.g., [\textit{CLS}] token in vanilla transformer\cite{vaswani2017attention}, \textit{Class Token} in ViT\cite{dosovitskiy2020image}, TNT\cite{han2021transformer}). During the experiment, we adopt our word-level transformer structure. The further discussion and comparison experiments of four different semantic information extractors are listed in the Appendix.
% % 我们的加权相加能显著减少需要传递给下游的参数数量，并能取得相同的表现能力
% 2) The attention-weighted sum can significantly reduce the number of features that need to be processed by the downstream component and achieve equivalent performance.

\textbf{Document-level Transformer:}
After obtaining the type-specific representation of each document, we adopt a document-level Transformer in the second stage of SIE Block to encode the representations for proposals. Given $A$'s document set $D = \{d_1, d_2, ... ,d_{|T|}\}$, we can obtain all the documents' representations set $\hat{\mathbf{e}}^{(l-1)}_D=\{\hat{e}^{(l-1)}_{d_1}, \hat{e}^{(l-1)}_{d_2}, ... ,\hat{e}^{(l-1)}_{d_{|T|}}\}$ from the previous step. Then, we put the documents' embeddings set to the document-level Transformer in layer $l$: 

\begin{equation}
\begin{aligned}
    \mathbf{e}^{(l)}_{D} & = \{e^{(l)}_{d_1}, e^{(l)}_{d_2}, ..., 
    e^{(l)}_{d_{|T|}}\} \\
    &= {Transformer}_{d}(\hat{\mathbf{e}}^{(l-1)}_D), 
\end{aligned}
\end{equation}
where ${Transformer}_{d}(\cdot)$ is a Transformer to extract the document-level features for proposals, $\mathbf{e}^{(l)}_{D} = \{e^{(l)}_{d_1}, e^{(l)}_{d_2}, ..., e^{(l)}_{d_{|T|}}\}$ is the Transformer outputs, which can be reviewed as $T$-views of representations for proposals. Contributed by the self-attention mechanism in Transformer, each document representation in the inputs can collect information from the context documents with different attention weights, so the corresponding output contains the information of the whole document set, which can be regarded as a facet of representation for proposals. 
% If there are multi-layer SIE, the $\Hat{e}^t_i$ will be assign to the next layer's $e^t_i$ as a vector representation of type token $t_i$.

Then we can give a formal definition of the input and output of SIE component as:\note{}
\begin{equation}
\begin{aligned}
    \mathbf{e}_D &= \{e_{d_1}, e_{d_2}, ..., e_{d_{|T|}}\} \\
    &= N_e \times SIEBlock(\mathbf{W}^{(0)}),
\end{aligned}
\end{equation}
where matrix $\mathbf{e}_D$ is the final output of SIE, represent the semantic information and multiple type information within the document set $D$. $\mathbf{W}^{(0)}=\{\mathbf{w}^{(0)}_1, \mathbf{w}^{(0)}_2, ..., \mathbf{w}^{(0)}_{|T|}\}$ is the initial word embedding of each documents in $D$. \note{component discussion is aborted}
\iffalse
Be noted that the SIE is a textual feature extractor essentially. 
We design the SIE in the consideration of both efficiency and effectiveness, which mainly has the following advantages:
% 1、利用attention机制，在word-level中，我们希望SIE能够在文章语句中发现能够为申请书分类的重要词汇，从而为下游分类提供更有效的语义信息。
% 2、虽然目前我们利用的raw data大多是属于短文本（200字以内），我们希望在面对申请书全文或者更多长文本数据时，模型能够有着更好的扩展性，所以我们在document-level中使用了一个线性变换模块以及相加模块来减少向下游传递的字符表征数。
% 3、在document-level中，我们利用self attention机制来捕捉针对特定类别的表征以及在申请书中他们的相互关系，我们希望不同类别的文本能够结合其他类型文本的表征来得到特定的表达。例如不同的关键词在不同的标题的申请书中可能有着不同的含义。
(1) Using the attention mechanism in word-level transformer, we hope that SIE can adaptively find critical characters in the sequence of the words, thus improving the classification of the proposal by providing more effective semantic information.
(2) We hope that the model can have better scalability when facing the full text of the proposal or more long text data. So we use a linear transform operation followed by an element-wise addition at the document-level transformer to both reduce the number of character representations passed downstream and combine the type-specific information.
(3) In the document-level Transformer, we use the self-attention mechanism to capture the representations with specific type information and their interrelationships in the proposals. We hope that the model can combine different text types with other text types to get particular expressions. (E.g., keywords may have different meanings in proposals with different titles.)
\fi
\iffalse
(1) Comparing with other RNN-like models as text encoder, Transformer is more efficient to learn the long-range dependencies between each word. 
Specifically, with the help of two-level Transformer encoder, we can obtain the associated proposal representations with long-range dependencies in both the word-level and the document-level. 
(2) Also, RNN-like models extract text information via sequentially propagation on sequence, which need serial operation of the time complexity of sequence length. While self-attention layers in Transformer connect all positions with constant number of sequentially executed operation. Therefore, Transformer can encoder text in paraller.
(3) The types of different textual features of proposals are taken into consider via adding the type-token in proposals' documents, which helps Transformer to extract type-specific outputs of documents. The design of two-level Transformers reduces the number of parameters of the encoder, which greatly improves the training efficiency of the entire model.
\fi

\subsubsection{Interdisciplinary Knowledge Extractor}
\note{As we aim to infer the Interdisciplinary label, the relations between disciplinary need to be incorporated. The disciplinary tree only contains single disciplinary information, thus, we introduce the co-word graph.}


\begin{figure}
\centering
\includegraphics[width=0.48\textwidth]{figure/encoder_2.eps} 
\caption{\textit{Interdisciplinary Knowledge Extractor}. The grey shading separates different components in IKE. The different colors of the node in $\mathbb{L}_{<k}$ and sub-graph represent different disciplines. The red outline on the node mark the central node. The $\hat{\mathcal{G}}_i$ is the sub-graph in $\mathcal{G}$ sampling by the chosen central node in $L_i$ with $Ng$ hops.}
\label{Fig.model_encoder_2}
\end{figure}


In the previous section \ref{co}, we utilized the co-word analysis theory to construct a Interdisciplinary Graph $\mathcal{G}$ to represent the relationship between disciplines. In this section, we propose the \textit{Interdisciplinary Knowledge Extractor} (IKE) on the Interdisciplinary Graph to capture the information of the interdisciplinary relationship of disciplines with others for helping the classification of potential interdisciplinary proposals.

% deleted by ziyue
%In the previous section \ref{co}, we utilized the co-word analysis theory to construct a Co-topic Graph $\mathcal{G}$ to represent the interaction between each discipline and represent the interdisciplinary relationship. To capture the inter-disciplinary knowledge from the hierarchical discipline system, we propose the \textit{Interdisciplinary Knowledge Extractor} (IKE), which is designed to obtain the co-occurrence information of the topic between each discipline.

Specifically, as illustrated in Figure \ref{Fig.model_encoder_2}, suppose given the sequence of label sets $\mathbb{L}_{<k}$ generated from previous $k-1$ steps prediction as input, where $\mathbb{L}_{<k} = [L_{0}, L_1,..., L_{k-1}]$, where each label set $L_i=\{l_i^j\}_{j=1}^{|L_i|}$ holds the $i$-th prediction result and is composed of a set of discipline labels. we aim to learn the interdisciplinary knowledge of each $L_i$ with other disciplines on the Interdisciplinary Graph $\mathcal{G}$. 
We conduct IKE, which consists of a multi-layer Graph Convolution Networks and a \textit{Readout} layer (the detail of GCNs is introduced in \ref{})\note{appedix}, on the sub-graphs of the nodes in input labels set $L_i$ in $i$-th level and integrate the neighborhood information on $G$ as the interdisciplinary knowledge into level-specific set embeddings $e_{L_i}$.

We first treat each discipline label in every set as a central node and sample its $N_g$-hops sub-graph from $\mathcal{G}$, where the $N_g$ is the layer number of GCNs. Then we pass the sub-graph set $\hat{\mathcal{G}}_{<k}=\{\hat{\mathcal{G}}_0, \hat{\mathcal{G}}_1,...,\hat{\mathcal{G}}_{k-1}\}$ and their node feature into $N_g$ layers of GCNs and a \textit{Readout} layer to obtain $e_{L_i}$:
\iffalse
\begin{equation}
\begin{aligned}
    \mathcal{H}^{N_g}_i &= N_g \times GCNLayer(\hat{\mathcal{G}}_i, \mathcal{H}^{0}_i),\\
    e_{L_i}& = Readout(\mathcal{H}^{N_g}_i, L_i),
\end{aligned}
\end{equation}
\fi
\begin{equation}
\begin{aligned}
    \mathcal{H}^{(N_g)}_i &= N_g \times GCNLayer(\hat{\mathcal{W}}_i, \hat{\mathcal{H}}^{(0)}_i),\\
    e_{L_i}& = Readout(\mathcal{H}^{(N_g)}_i, L_i),
\end{aligned}
\end{equation}
where the $\hat{\mathcal{H}}^{(0)}_i $ is the random initialized features of each node in sub-graph $\hat{\mathcal{G}}_i$ and the $\hat{\mathcal{W}}_i$ is the weighted adjacency matrix of $\hat{\mathcal{G}}_i$. The $\mathcal{H}^{(N_g)}_i$ is a hidden output matrix undergoing $N_g$ times GCN layers propagate on the sub-graph. The \textit{Readout} layer is to get the representation of the central nodes from $\mathcal{H}^{(N_g)}_i$, which can be a lookup operation, a mean pooling operation, or a self-attention layer\cite{lee2019self}, etc. For simplicity, we set the readout as a mean pooling operation after a lookup operation via the index of nodes in $L_i$ on $\mathcal{H}^{(N_g)}_i$. The $e_{L_i} \in \mathbb{R}^h$ is the final representation of $i$-th label set $L_i$. Then we can form the representation of sequence of label set $\mathbb{L}_{<k}$ as $\mathbf{e}_{\tiny \mathbb{L}_{<k}}=[e_{\tiny L_0}, e_{\tiny L_1},...,e_{\tiny L_{k-1}}]$. The $\mathbf{e}_{\tiny \mathbb{L}_{<k}}$ can be seen as the representation of the prediction result from the previous $k-1$ step integrated with related interdisciplinary knowledge.
\iffalse
The IKE aims to aggregate interdisciplinary relationship of each disciplinary in the predicted label sets in each level. We believe the characteristic of graph convolution network can help the model better understand the interaction between each discipline and initial an interdisciplinary knowledge-based representation of each level's disciplines for the rest process.
\fi

% deleted by ziyue
%The IKE will first treat the node in input labels set as the central node and save the \textit{Co-occurrence} neighborhood information to its sub-graph from Co-topic graph $\mathcal{G}$. Then, the Graph Convolution Networks in IKE will integrate the information between the central nodes and their neighborhood node (see Equation \ref{gcn1},\ref{gcn2}) as interdisciplinary knowledge. After a \textit{Readout} layer, the sequence of nodes embedding sets turns to the sequence of set embeddings to hold the knowledge within the central node among each sub-graphs. 

% deleted by ziyue
%Specifically, the prediction results in $\mathbb{L}_{<k}$ from the previous $k-1$ step can be viewed as a sequence of label set. Each label set $L_i=\{l^i_j\}_{j=1}^{|L_i|}$ holds the $i$-th prediction result and is composed of the discipline labels. 

% deleted by ziyue
\iffalse
In the first step of IKE, we treat each discipline label in every set as a central node and sample its $N_g$-hops sub-graph from $\mathcal{G}$, where the $N_g$ is the layer number of GCNs. Then we pass the sub-graph set $\hat{\mathcal{G}}_{<k}=\{\hat{\mathcal{G}}_0, \hat{\mathcal{G}}_1,...,\hat{\mathcal{G}}_{k-1}\}$ and their node feature into $N_g$ layers of GCNs to obtain the representation of each central node:
\begin{equation}
    \mathcal{H}^{N_g}_i = N_g \times GCNLayer(\hat{\mathcal{G}}_i, \mathcal{H}^{0}_i),
\end{equation}
where the $\mathcal{H}^{0}_i $ is the initial feature of each node in sub-graph $\hat{\mathcal{G}}_i$. The $\mathcal{H}^{N_g}_i$ is a matrix undergoing $N_g$ times GCN layers propagate, which represents the interdisciplinary knowledge in each node from label set $L_i$ and their neighborhood knowledge within $N_g$ hops. 

After extracting the interdisciplinary knowledge among each labels' neighborhood sub-graph, we use a \textit{Readout} layer to get the representation of each sub-graph by the central node information. In detail, the process is defined as:
\begin{equation}
    e_{L_i} = Readout(\mathcal{H}^{N_g}_i, L_i),
\end{equation}
where $e_{L_i} \in \mathbb{R}^h$ is the final representation of $i$-th label set $L_i$. Then we can form the representation of sequence of label set $\mathbb{L}_{<k}$ as $\mathbf{e}_{\tiny \mathbb{L}_{<k}}=[e_{\tiny L_0}, e_{\tiny L_1},...,e_{\tiny L_{k-1}}]$. The $\mathbf{e}_{\tiny \mathbb{L}_{<k}}$ can be seen as the representation of the prediction result from the previous $k-1$ step with related interdisciplinary knowledge.

The IKE aims to aggregate node representation from each central node's neighborhood sub-graph on Interdisciplinary Graph. We believe the characteristic of graph convolution network can help the model better understand the interaction between each discipline and initial an interdisciplinary knowledge-based representation of each discipline for the rest process. 
% In addition, the embedding of the results of the previous step can initial at any level, which gives the model the ability to derive from an arbitrary-granularity label sequence to the finest-grained label sequence. In other words, the IKE can utilize the guidance labels provided by experts in reality to generate more fine-grained results.
\fi
\begin{figure}
\centering
\includegraphics[width=0.48\textwidth]{figure/Decoder.eps} 
\caption{\textit{Information Fusion} and \textit{Level-wise Prediction} in step-$k$. }
% The left side of this figure illustrate the structure of Information Fusion component. The input is the information from previous $k-1$ step prediction and the semantic information of research proposal extracted from SIE. After $N_d$ times iteration of IF Block process, we can obtain the fusion matrix $\mathbf{S}_k$. The right side is the Level-wise prediction component, which will utilize the hierarchical information from hierarchical discipline structure $\gamma$ and the fusion matrix $\mathbf{S}_k$ to generate step-$k$ prediction results.
\label{Fig.model_decoder}
\end{figure}
\subsection{Information Fusion}
In \textit{Information Fusion} (IF), we aim to integrate the semantic information and previous prediction results with disciplinary knowledge. As you can see in the left side of Figure \ref{Fig.model_decoder}, the IF's structure is based on \textit{Multi-Head Self-Attention Mechanism} \note{appedix}
% in Equation \ref{eq:3}-\ref{eq7}
, which is consisted with multiple IF Block layers. The first part of IF aims to extract the ancestor label information of $\mathbb{L}_{<k}$ and learn the dependency of labels on the hierarchical discipline structure. And the rest is design to integrate the proposal representations and ancestor label information via the attention layer.
\iffalse
In \textit{Information Fusion} (IF), we aim to integrate the semantic information and previous prediction results with disciplinary knowledge. As you can see in the left side of Figure \ref{Fig.model_decoder}, the IF's structure is based on \textit{Multi-Head Self-Attention Mechanism}  in Equation \ref{eq:3}-\ref{eq7}, which is consisted with multiple IF Block layers, its architecture is similar to the SIE, but it introduce a source attention layer in addition to the self-attention layer. The first part of IF aims to extract the ancestor label information of $\mathbb{L}_{<k}$ and learn the dependency of labels on the hierarchical discipline structure. And the rest is design to integrate the proposal representations and ancestor label information via the attention layer.
\fi
Formally, from the IE, we can obtain the representation of former prediction result with interdisciplinary knowledge $\mathbf{e}_{\tiny \mathbb{L}_{<k}}$. We sum the embedding with corresponding positional embeddings as the input $\mathbf{S}^{(0)}_{\tiny <k}=\{s^{(0)}_{root},s^{(0)}_{1},s^{(0)}_{2},...,s^{(0)}_{k-1}\}$ of first stage of IF:
\begin{equation}
\begin{aligned}
    \label{pe}
    \mathbf{S}_{<k}^{(0)}=PE(\mathbf{e}_{\tiny \mathbb{L}_{<k}}),
\end{aligned}
\end{equation}
where $PE(\cdot)$ is the positional encoding function.

After that, given $\mathbf{S}^{(l-1)}_{\tiny <k}$ and semantic information $\mathbf{e}_D$, the propagation of the $l$-th layer in the IF is defined as:
\begin{equation}
\label{M}
    \hat{\mathbf{S}}_{<k}^{(l-1)} = \sigma( \mathbf{S}_{<k}^{(l-1)}+ MultiHead(\mathbf{S}_{<k}^{(l-1)},\mathbf{S}_{<k}^{(l-1)},\mathbf{S}_{<k}^{(l-1)})),
\end{equation}

% The second stage of IF is a source attention component:

\begin{equation}
\label{Z}
    Z^{(l-1)} = \sigma(\hat{\mathbf{S}}_{<k}^{(l-1)} + MultiHead(\hat{\mathbf{S}}_{<k}^{(l-1)} , \mathbf{e}_D, \mathbf{e}_D)),
\end{equation}

\begin{equation}
\label{L}
    \mathbf{S}_{<k}^{(l)} =  \sigma(Z^{(l-1)}+\mathcal{F}(Z^{(l-1)})),
\end{equation}
where the propagation can be divided into two stages. In Equation \ref{M}, the input label is feeded into a multi-head self-attention layer to capture the dependency between labels in the label set, and the output $\hat{\mathbf{S}}_{<k}^{(l)} \in \mathbb{R}^{k\times h}$ preserves the ancestor labels information, which is utilized in the second stage. In Equation \ref{Z} and \ref{L}, $\hat{\mathbf{S}}_{<k}^{(l)}$ is incorporated with the proposal representation matrix $\mathbf{e}_D$ via a source attention layer, where $\hat{\mathbf{S}}_{<k}^{(l)}$ is the query, $\mathbf{e}_D$ is the key and value, which aims to extract information from the proposal corresponding to the predicted labels. The output of this layer is the hidden embeddings $\mathbf{S}_{<k}^{(l)} =[s^{(l)}_{root},s^{(l)}_{1},s^{(l)}_{2},...,s^{(l)}_{k-1}]$, where each $s^{(l)}_i$ can be seem as a representation of the proposal which is correlated with the label $l_i$. 
Finally, We stack $N_d$ layers of above components and obtain the final output in last layer:
% = \mathbf{S}_{<k}^{(N_d)}
\begin{equation}
\begin{aligned}
    \mathbf{S}_{k} &  = [s^{\tiny(N_d)}_{root},s^{\tiny (N_d)}_1,s^{\tiny (N_d)}_2,...,s^{\tiny (N_d)}_{k-1}] \\
    &=N_d \times IFBlock(\mathbf{e}_{\tiny \mathbb{L}_{<k}}, \mathbf{e}_D)
\end{aligned}
\end{equation}
where $\mathbf{S}_{k}\in \mathbb{R}^{k\times h}$ is the fusion matrix that integrated the proposal information with $k$ previous ancestor labels of the proposal, which can be seen as $k$ proposal representations corresponding to the $k$ levels with interdisciplinary knowledge. And $N_d$ is the total layer number of IF Block.

\subsection{Level-wise Prediction}
According to Equation \ref{equation_1}, we hope that the HMDG can generate labels set in a top-down fashion from the beginning level to a proper level $H_A$ obey the hierarchical discipline structure $\gamma$ step by step, with considering both the proposal's semantic information in documents set $D$ and the obtained ancestor label set sequence $\mathbb{L}_{<k}$'s interdisciplinary knowledge $\mathcal{G}$. 
The right side of Figure \ref{Fig.model_decoder} demonstrate the prediction in step-$k$. We first feed the fusion matrix $\mathbf{S}_{k}$ into a pooling function, a fully connected layer and a Sigmoid layer to generate each label's probability for $k$-th level-wise label prediction.
\begin{equation}
 {\hat{y}}_k= Sigmoid({\mathcal{F}}_{k}(Pooling(\mathbf{S}_{k}))),
\end{equation}
where $\hat{y}^i_k\in [0,1]$ is the predicted probability of the $i$-th discipline $c^i_k$ in level-$k$ $c^i_k \in C_k$. The $\mathcal{F}_{k}(\cdot)$ denotes a level-specific feed-forward network with ReLU activation function to project the input to a $|C_k|+1$ length vector. 
After the $Sigmoid(\cdot)$, the final output $\hat{y}_k$ is the probability of $k$-th level's labels. 
In prediction progress, the label corresponding to the index of the value in the $\hat{y}_k$ that achieves the threshold will be selected to construct the current prediction result.
In our paper, we set this pooling operation as directly taking the last vector of $\mathbf{S}_{k}$, as its level is the most is the closest to the level $k$ where the label needs to be predicted. 
Noted that we require that the model is able to define a distribution over labels of all possible lengths, we add a end-of-prediction label $l_{stop}$ to all levels, and set the last element of the probability in each level is the probability of label $l_{stop}$. In each label path's last step, the $l_{stop}$ is the prediction result, the prediction process should end in the level-$H_A$ and output the current predicted labels as the final result. Thus, the level-$k$'s
objective function $\mathcal{L}_k$ can be defined as:

\begin{equation}
\begin{aligned}
    \mathcal{L}_k(\Theta)    &= \log(P(L_k|D,\gamma,\mathcal{G},\mathbb{L}_{<k}; \Theta))\\
     &= \sum^{|C_k| + 1}_{i=1} \left(y_i \log(\hat{y}_k^i) + (1 - y_i) \log(1 - \hat{y}_k^i) \right) \\
\end{aligned}
\end{equation}
where the $L_k$ is the ground truth label set of level-$k$ prediction. And $y_i=\mathbbm{1}(l_i \in L_k)$, which aims to discriminate whether the $i$-th label $l_i$ belongs to the truth label set or not.  
Finally, after the prediction from level-$1$ to level-$H_A$, the overall objective function for each proposal $A$ with document set $D$ is to maximize the log-likelihood of the overall probability:
\begin{equation}
        \Theta = \mathop{\arg\max}_{\Theta}\sum_{k=1}^{H_A} \log P(L_k|D,\gamma,\mathcal{G},\mathbb{L}_{<k}; \Theta)
\end{equation}

% \begin{equation}
% s.t. \space y_i = \mathbbm{1}(l_i \in L_k), 
% \end{equation}
% P(L_k|D,\gamma,\mathcal{G},\mathbb{L}_{<k}; \Theta) = \prod_{i=1}^{|L_k|}\hat{y}_{k,i}
% \end{equation}
\iffalse
\note{mention the stop label}
\note{check}
To summarize, the HMDG is a knowledge-guided hierarchical multi-label multi-document classification model. The design of the model is based on a real-world scenario. The main advantage of HMDG architecture is summarized as follow: 
(1) We design the Semantic Information Extractor component to capture the information on each document fully. Further, we propose the Interdisciplinary Knowledge Extractor to help the model predict the interdisciplinary proposal more precisely.
(2) We introduce the Transformer model into HMDG by utilizing its proven superior performance in aligning the semantic and syntactic information in the translation model. Our motivation is to analogy the hierarchical discipline structure as the target language, then use the Transformer decoder structure in the Information Fusion component to capture the dependency information.
(3) By introducing the end-of-prediction label $l_{stop}$, the HMDG gained the capacity of predicting the label length of the proposal, which means the decoder can automatically learn the proper granularity of discipline for proposals.\note{from icdm}
(4) Unlike other HMC models, we introduce the previous prediction results by transferring explicit symbolic information. Thus, in the real-world scenario, HMDG can use the previous prediction results to generate the rest prediction label, which gives the model ability to start prediction at any level and can aid the scientists to finish the most fine-grained labels.\note{experiment to proof}
\fi



\subsubsection{Document-level Transformer:}
Then, we use a fully-connected layer to transform the vectorized vanilla document representation to a vector. Next, the vector will element-wise add with its \textbf{type-token} vector to get the type-specific representation $\hat{e}^{(l-1)}_{d_i}$:

\begin{equation}
\label{ew2}
    \begin{aligned}
    \hat{e}^{(l-1)}_{d_i}=e^{(l-1)}_{d_i} + FC(Vec(\mathbf{w}^{(l)}_{i})),
\end{aligned}
\end{equation}

Then, we obtain the type-specific documents' representations set  $\hat{\mathbf{e}}^{(l-1)}_D=\{\hat{e}^{(l-1)}_{d_1}, \hat{e}^{(l-1)}_{d_2}, ... ,\hat{e}^{(l-1)}_{d_{|T|}}\}$, we put it into a document-level Transformer to aggregate the contextual information between documents:

\begin{equation}
\begin{aligned}
    \label{trans2}
    \mathbf{e}^{(l)}_{D} = {Transformer}_{d}(\hat{\mathbf{e}}^{(l-1)}_D), 
\end{aligned}
\end{equation}
where ${Transformer}_{d}(\cdot)$ is a Document-level Transformer, $\mathbf{e}^{(l)}_{D}\in \mathbb{R}^{|T| \times h}$ is the outputs, which can be seen as $|T|$-views of high-level abstraction for proposals.

==> document/preliminaries_old.tex <==
In this section,  we start by giving the definition to the research proposal, the hierarchical discipline structure, and the interdisciplinary graph. Then, we propose a formal definition of the Interdisciplinary Proposal Classification (IPC) problem. 
% \begin{table}
% \centering
% \caption{Main Symbol Table}
% \begin{tabular}{l|l} 
% \hline
% Notations & Descriptions  \\ 
% \hline
%   $A$          & the research proposal\\
%   $D$          & the document set of $A$\\
%   $d_i$          & the type $t_i$ document in $D$\\   
%   $T$          & the type set of each documents\\ 
%   $t_i$          & the type of the $d_i$ in the $D$\\
%   $w^i_j$          & the $j$-th word token in $i$ type document $d_i$\\
%   $\gamma$     & the hierarchical discipline system\\
%   $H$          & the total level number of $\gamma$\\
%   $\mathbb{C}$ & the set of discipline labels on $\gamma$\\
%   $C_i$        & the $i$-th level of discipline labels set on $\gamma$\\
%   $c$          & the discipline label\\
%   $\prec$      & the \textit{Belong-to} relation between two $c$\\
%   $L$ & the length-variant sequence of label set of $A$\\
%   $H_A$    & the total level number of $A$. also is the length of $L$\\
%   $R$ & the co-topic relation edge set between each $c$\\
%   $r_{{c_i},{c_j}}$ & the co-topic edge between $c_i$ and $c_j$\\
%   $w^r_{{c_i},{c_j}}$ & the weight of the co-topic edge $r_{{c_i},{c_j}}$\\
  
% \hline
% \end{tabular}
% \end{table}

\subsection{The Research Proposal}
The scientist or the researcher commits the research proposal to apply for research funding. In general, each proposal is carefully written and combines multiple texts representing the insightful idea associated with a few topics in one or two disciplines. Like the toy example in Figure \ref{Fig.label_1}(1), a proposal may have multiple textual characteristics, including \textit{Title}, \textit{Abstract}, and \textit{Keywords}, etc. We collect the text information of these characteristics as documents and orderly compose these documents of each proposal together to a document set. 
Formally, a proposal is expressed as $A$, the document set of $A$ is $D=\{d_1, d_2,...,d_{|T|}\}$ and their types are marked by $T =\{t_1,t_2,...,t_{|T|}\}$. The $|T|$ is number of document types, and $d_i$ is the document with type $t_i$.  Every document $d_i$ in the proposal, denoted as $d_i=[w^{1}_i,w^{2}_i,...,w_{i}^{|d_i|}]$, is consists of a sequence of words $w^{k}_i$, which denotes the $k$-th word in the $i$ type of document. 

\subsection{Hierarchical Discipline Structure}\label{d1}

The hierarchical discipline structure, expressed as $\gamma$, is a DAG or a tree that is composed of discipline entities and the \textit{Belong-to} relation from a discipline to its sub-disciplines. On $\gamma$, the discipline nodes can be treated as a group of topics or knowledge from a particular domain. The links between each discipline node are uniform and directed, pointing from parent nodes to the child nodes, and the child node is a sub-discipline of the parent node. 

Formally, the node on this tree is organized in $H$ hierarchical levels $\mathbf{C}=(C_0, C_1,C_2,...,C_H)$, where $|\mathbf{C}|$ is the total number of disciplines, and $H$ is the total depth of hierarchical level. $C_i=\{c^1_i,c^2_i,...,c^{\tiny |C_i|}_i\}$ is the set of the disciplines in the $i$-th hierarchical level and $|C_i|$ is the total number of disciplines in $C_i$. The $C_0=\{root\}$ is the root level of $\gamma$. In order to describe the connection between different disciplines, we introduce $\prec$, a partial order representing the \textit{Belong-to} relationship. $\prec$ is asymmetric, anti-reflexive and transitive\cite{wu2005learning}:
\begin{small}
 \begin{align} 
   & \bullet \text{The only one greatest category }\textit{root}\text{ is the root of the } \gamma,  \nonumber\\
   % root是所有节点的起点
   & \bullet \forall c^x_i \in C_i, c^y_j \in C_j, c^x_i \prec c^y_j \to \space c^y_j \not\prec c^x_i,  \nonumber\\
   % 关系不是对称的
   & \bullet \forall c^x_i \in C_i, c^x_i \not\prec c^x_i, \nonumber\\
   %自身不包含
   & \bullet \forall c^x_i \in C_i, c^y_j \in C_j, c^z_k \in C_k, c^x_i \prec c^y_j \land c^y_j \prec c^z_k \to c^x_i \prec c^z_k.  \nonumber
   % 关系可以传递
   \nonumber
 \end{align}
\end{small} 
Finally, we define the Hierarchical Discipline Structure $\gamma$ over $\mathbf{C}$ as a partial order set $\gamma=(\mathbf{C},\prec)$.
% \end{definition}

% \begin{definition}[\textbf{Co-topic Graph}]
\subsection{Interdisciplinary Graph} 
% \note{reorganize, try to illustrate the impact of two component, and give a name to this measure.
% like low freq x high overlap $\to$ A type, high freq x high overlap $\to$ big impact, high freq x low overlap$\to$biggest impact, low freq x low overlap$\to$little impact}
\label{co}
% 在涉及到交叉学科的分类问题，很自然的对于学科标签的特征建模
% The co-topic graph is composed of a set of discipline labels and the \textit{Co-occurrence} relation between each label. According to definition \ref{d1}, the discipline is a combination of the domain knowledge and topics. Further, the topic of each proposal is carefully selected~\cite{he1999knowledge} and proposed by the scientists and denoted by the \textit{Keywords} text. 
% Suppose we have a set of proposals $\mathbb{A}=\{A_1, A_2,..., A_{|\mathbb{A}|}\}$, for each proposal $A_i$ we have its related \textit{Keywords} set $K_i=\{k_i^1, k_i^2,...,k_i^{|K_i|}\}$ and the related discipline labels set $L_i=\{l_i^1,l_i^2,...,l_i^{|L_i|}\}$, where each label $l_i^j$ in $L_i$ represent a node on discipline set $\mathbb{C}$. Then, we can group the \textit{Keywords} of each proposal into the discipline node set $\mathbb{C}$ by the label $l$. 
% After, we extract the \textit{Co-occurrence} relation between each discipline by the selection of the keywords and its overlap on each proposal. 
The discipline is a combination of the domain knowledge and topics. Further, the topic of each proposal is carefully selected~\cite{he1999knowledge} and proposed by the scientists and denoted by the \textit{Keywords} text. 
% 1、为了更好的表示学科间的互动关系，我们构建了co-topic图。
% specifically，我们构建了一张权值图g=（V，E，w），利用w（A，B）表示一条位于两个学科间的有向边权值，也就是学科A对于学科B的主题的交汇情况。
% 学科图的主要组成是 V E w
By that, we construct a weighted graph to better represent the interdisciplinary relationship, capturing the cooccurrence tendency of the topic among each discipline.
% The recent approaches\cite{yao2019graph,Tang2020} use an undirected graph and Pointwise Mutual Information (PMI) to capture collocations and associations between words. However, these things are completely different when it comes to modeling the relationships between disciplines. 
From the disciplines' perspective, the interactive strength between two disciplines should not only be impacted by the frequency of co-topics that occur but also by the overlap topics each contains. 
% 交叉性-- 申请书的结合程度，研究主题的diversity
% 假设1: 申请书中共现程度越高的学科之间具有更高的交叉性
% 假设2: 学科研究主题重合度越高的学科之间具有更低的交叉性
\note{qzy: From the disciplines' perspective, the interactive strength between two disciplines is not only be related to the amount of overlapping topics between them, but also related to the proportion of topic overlapping frequency of each discipline.}
% We demonstrate the four situations of the interdisciplinarity strength between two disciplines in Table \ref{co-topic demo}.
% \begin{table}
% \caption{}
% \centering
% \resizebox{0.95\linewidth}{!}{%
% \begin{tabular}{c|c|c} 
% \hline
%                                   & \makecell[c]{Low Percentage of\\Topic Overlap} & \makecell[c]{High Percentage of\\Topic Overlap}                 \\ 
% \hline
% \makecell[c]{High Frequency of\\Co-topic Happend} & Strong Interdisciplinarity      & \makecell[c]{Subordinate Discipline \\Or Similar Discipline}    \\ 
% \hline
% \makecell[c]{Low Frequency\\of Co-topic Happend}  & Weak Interdisciplinarity        & \makecell[c]{Inner-disciplinary\\Interdisciplinarity Or Other}  \\
% \hline
% \end{tabular}}
% \label{co-topic demo}
% \end{table}
Thus, the \textit{Interdisciplinary Graph} should be a directed graph, and the weight of edges from the source discipline to the destination should be different from its reverse edge.
For the reasons above, We adopt a nonparametric quantitative heuristic named \textit{Rao-Stirling} (RS) measure~\cite{stirling2007general} to construct the graph and calculate the value of adjacency matrix $\mathcal{W}$ by identifying relationships and interactions between the disciplines~\cite{gomez2016handbook}.
The RS is widely adopted to measure the diversity of the discipline system~\cite{stirling2007general,porter2009science,rafols2010diversity}, ecosystem~\cite{biggs2012toward} and energy security~\cite{winzer2012conceptualizing} which is defined as: 
\begin{equation}
\label{rs}
Diversity = \sum_{ab(a \not = b)} (p_a\cdot p_b)^\alpha \cdot (dist(a,b))^\beta,
\end{equation}
where the first part of Equation \ref{rs} is the probability distributions ($p_a$ and $p_b$) of the units of analysis, and the rest $dist(a,b)$ is the distance between the $a$ and $b$. The $\alpha$ and $\beta$ are two constant to weighting the two components. 

%Specifically, we build the \textit{Interdisciplinary Graph} denoted as $\mathcal{G}=(\mathcal{C}, E)$, where $\mathcal{G}$ is a collection of discipline nodes $\mathcal{C}=\left\{c_i\right\}^{|\mathbb{C}|}_{i=1}$ and directed \textit{Co-occurence} edges $E=\left\{e_{a\to b}\right\}^{|\mathbb{C}|}_{a,b=1}$. 
%The adjacency matrix $\mathcal{W}$ of graph $\mathcal{G}$ contains non-negative weights associated with each edge: $\mathcal{W}_{a\to b}\ge 0$. If there is no \textit{Co-occurence} relation from $c_a$ to $c_b$, then $\mathcal{W}_{a \to b}=0$. Inspired by the RS, we introduce the RS to a micro view named $\mathcal{W}_{a \to b}$ to measure the weight of edge from discipline $a$ to discipline $b$:
\note{qzy: 
Specifically, we build the \textit{Interdisciplinary Graph} denoted as $\mathcal{G}=(\mathcal{C}, E)$, where $\mathcal{G}$ is a collection of discipline nodes $\mathcal{C}=\left\{c_i\right\}^{|\mathbb{C}|}_{i=1}$ and directed \textit{Co-occurence} edges $E=\left\{e_{a\to b}\right\}^{|\mathbb{C}|}_{a,b=1}$. Each $e_{a\to b}$ represents the edge from discipline $c_a$ to discipline $c_b$ and is associated with the weight $\mathcal{W}_{a\to b}\ge 0$. 
We introduce the RS in a micro view to measure $\mathcal{W}_{a\to b}$:
}
\begin{equation}
    \mathcal{W}_{a \to b} = (p_{a\to b})^\alpha (dist(a\to b))^\beta,
\end{equation}
%where, in our paper, we set $\alpha$ and $\beta$ as 1. The first part of $\mathcal{W}$ is $(p_{a\to b})^\alpha$, which indicate the co-word frequency between two discipline $a$, $b$, and all their sub-diciplines. The second part of $\mathcal{W}$ is the overlap between two discipline, and all their sub-diciplines.
\note{qzy: where $\mathcal{W}_{a \to b}=0$ if there is no \textit{Co-occurence} relation from $c_a$ to $c_b$, and in our paper, we set $\alpha$ and $\beta$ as 1. }
%Thus, we can obtain the non-negative adjacency matrix $\mathcal{W}$ of graph $\mathcal{G}$. 
%The first part of $\mathcal{W}$ is $(p_{a\to b})^\alpha$, which indicate the co-word frequency between two discipline $a$, $b$, and all their sub-diciplines. The second part of $\mathcal{W}$ is the overlap between two discipline, and all their sub-diciplines,
The $p_{a\to b}$ and $dist(a\to b)$ are defined as:

\begin{equation}
    p_{a\to b} = \frac{\sum_{i}^{n} \mathbbm{1}(k_i \in \{K_a \cap K_b\})K_a[k_i]}{\sum_{i}^{n}K_a[k_i]},
\end{equation}
\begin{equation}
    dist(a \to b) = 1 - \frac{|K_a \cap K_b|}{|K_a|},
\end{equation}

where $p_{a\to b}$ represents the probability of co-word frequency 




%In order to represent the disciplinary similarity, we further improve the components in RS by:
% w的计算形式是利用了共词分析的思路，通常xxx，PMI，共词方法xxx，
% 不过在学科Interdisciplinary的构建过程中场景更具体。
% 例如学科A内包含大量的主题，而学科B包含少量主题，这种场景在上下级学科间会经常出现，这样学科A到学科B与学科B到学科A的权重应当是不同的，也就是如果学科A与学科B之间出现了共词的情况，那么少量主题的学科B对于大量主题的学科A的影响，应该相对小于大量学科主题学科A对于拥有少量主题的学科B的影响。
\begin{equation}
    p_{a\to b} = \frac{\sum_{i}^{n} \mathbbm{1}(k_i \in \{K_a \cap K_b\})K_a[k_i]}{\sum_{i}^{n}K_a[k_i]},
\end{equation}
\begin{equation}
    dist(a \to b) = 1 - \frac{|K_a \cap K_b|}{|K_a|},
\end{equation}
where the $dist(\cdot)$ is a distance function to stand for the difference on topic between two disciplines. The $p_{a,b}$ represent the probability  the proposal in $c_a$ that contains same topic in $c_b$. The $\mathbbm{1}(\cdot) \to \{0, 1\}$ is the indicator function, $K_a$ and $K_b$ are the look-up table of \textit{Keywords} and its frequency in discipline $c_a$ and $c_b$. $k_i$ is the $i$-th keyword in \textit{Keywords} set. $n$ is the total number of \textit{Keywords}. 





% 1、学科之间的关系和学科自身包含的主体数量，理论上来讲，主题数量越多的学科，与其他学科共同主题在其整体主题数量的占比就越小

% For example, discipline A contains more topics while discipline B contains less, which will often occur between discipline and its subdiscipline. 
% In this way, the impact of A to B should be higher than B to A. 
% In other words, if there is a \textit{Co-occurence} relationship between A and B, then B with a smaller number of topics should have a relatively more minor impact on A than that of A on B.



% The \textit{Co-topic Graph} is denoted as $\mathcal{G}=(V, E, \mathcal{W})$, where $\mathcal{G}$ is consist of the discipline node $V$, the \textit{Co-occurence} edges $E$ and the weight $\mathcal{W}$ of each edge. The weight $\mathcal{W}(e_i) \to w_i$ is the Pointwise Mutual Information (PMI) between two discipline. Formally, give two discipline $c_i$ and $c_j$, they have related keyword frequent set $K^f_{c_i}$ and $K^f_{c_j}$

% \begin{equation}
% \begin{aligned}
%     % p(c) &= \sum(f)\\
%     PMI(c_i, c_j)&=log\frac{p(c_i,c_j)}{p(c_i)p(c_j)}
% \end{aligned}
% \end{equation}

%=\left\{(k_1, f_1), (k_2, f_2),...,(k_n, f_n)\right\}


% cPMI
% 依据这个思路 。。。。 我们定义了xxxx， formally xxx A ：具体的定义方法
% 1、学科之间的关系和学科自身包含的主体数量，理论上来讲，主题数量越多的学科，与其他学科共同主题在其整体主题数量的占比就越小
% $$V=\left\{v_i\right\}^{|\mathbb{C}|}_{i=1}$$
% $$E=\left\{e_{i \to j}\right\}^{|\mathbb{C}|}_{i,j=1;i\not = j}$$
% $$\mathcal{W}(e_{a\to b}) = \frac{\sum_{i}^{n} \mathbbm{1}(w_i \in \{K_a \cap K_b\}) K_a[w_i]}{\sum_{i}^{n}K_a[w_i]}  $$

% \end{definition}



%\definition{HMPC Problem Definition} 
% \begin{definition}[\textbf{Hierarchical Multi-label Proposal Classification}]
%我们把每一个学科看作是label，那么这个问题的output就是输出一个set的label，L，且这个L满足。
\subsection{Interdisciplinary Research Proposal Classification}
Finally we provide a formal definition of IRPC task. Given a proposal $A$, we aim to extract its semantic informaion from the document set $D$ and assign multiple paths of discipline for it from the hierarchical discipline structure $\gamma$. By treating each discipline in $\gamma$ as a label, we can view this problem as assigning a sequence of label set for each input data. The disciplines in each label set belong to one of the paths in the hierarchy of $\gamma$, where each path is directional and started from the root node with arbitrary length.

Formally, the sequence of label set is denoted as $\mathbb{L} = [L_1, L_2,..., L_{H_A}]$, where $L_i=\{l_i^1, l_i^2, ..., l_i^{|L_i|}\}$ is a label set with arbitrary number of disciplines on $\gamma$, $\forall l_i^j \in L_i \to l_i^j \in C_i$. $H_A$ is the length of the sequence $\mathbb{L}$.
Moreover, we consider that the information of topic co-occurrence between each discipline is facilitated to interdisciplinary label assignment, so, we introduce the \textit{Interdisciplinary Graph} $\mathcal{G}$ to improve the model performance. 
Finally, IPC problem can be formulated as:
\begin{equation}
    \Omega(D,\gamma,\mathcal{G},\Theta) \to \mathbb{L}, \nonumber
\end{equation}
where $\Theta$ is the parameters of model $\Omega$. Figure 1 demonstrates a toy model of the IPC problem.

% \end{definition}


% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{figure/aggre_2.eps} 
% \caption{An example of the $\mathcal{G}$ in the view of a central node $c_a$. The thickness of the red arrows represents the weight on this directed edge. The grey dotted line is the structure of discipline system, and the different color of shading means different major disciplines.}
% \label{Fig.aggre}
% \end{figure}



==> document/table/all.tex <==
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{c|clcclc|cclcll}
\hline
\multirow{3}{*}{Baseline} & \multicolumn{6}{c|}{Level-1}                                                                                                                                                                                                      & \multicolumn{6}{c}{Level-2}                                                                                                                                                                                                   \\ \cline{2-13} 
                          & \multicolumn{3}{c|}{Micro}                                                                                      & \multicolumn{3}{c|}{Macro}                                                                                      & \multicolumn{3}{c|}{Micro}                                                                                      & \multicolumn{3}{c}{Macro}                                                                                   \\ \cline{2-13} 
                          & \multicolumn{1}{c|}{F1}             & \multicolumn{1}{c|}{P}              & \multicolumn{1}{c|}{R}              & \multicolumn{1}{c|}{F1}             & \multicolumn{1}{c|}{P}              & R                                   & \multicolumn{1}{c|}{F1}             & \multicolumn{1}{c|}{P}              & \multicolumn{1}{c|}{R}              & \multicolumn{1}{c|}{F1}             & \multicolumn{1}{c|}{P}              & \multicolumn{1}{c}{R}           \\ \hline
                          TextCNN                   & \multicolumn{1}{c|}{0.757}          & \multicolumn{1}{c|}{0.770}          & \multicolumn{1}{c|}{0.744}          & \multicolumn{1}{c|}{0.639}          & \multicolumn{1}{c|}{0.665}          & 0.618                               & \multicolumn{1}{c|}{0.512}          & \multicolumn{1}{c|}{0.553}          & \multicolumn{1}{c|}{0.477}          & \multicolumn{1}{c|}{0.426}          & \multicolumn{1}{c|}{0.491}          & \multicolumn{1}{c}{0.403}       \\
DPCNN                     & \multicolumn{1}{c|}{0.710}          & \multicolumn{1}{c|}{0.702}          & \multicolumn{1}{c|}{0.718}          & \multicolumn{1}{c|}{0.589}          & \multicolumn{1}{c|}{0.596}          & 0.586                               & \multicolumn{1}{c|}{0.429}          & \multicolumn{1}{c|}{0.439}          & \multicolumn{1}{c|}{0.420}          & \multicolumn{1}{c|}{0.357}          & \multicolumn{1}{c|}{0.368}          & \multicolumn{1}{c}{0.358}       \\
FastText                  & \multicolumn{1}{c|}{0.762}          & \multicolumn{1}{c|}{0.765}          & \multicolumn{1}{c|}{0.758}          & \multicolumn{1}{c|}{0.646}          & \multicolumn{1}{c|}{0.655}          & 0.639                               & \multicolumn{1}{c|}{0.517}          & \multicolumn{1}{c|}{0.543}          & \multicolumn{1}{c|}{0.493}          & \multicolumn{1}{c|}{0.430}          & \multicolumn{1}{c|}{0.476}          & \multicolumn{1}{c}{0.420}       \\


TextRNN                   & \multicolumn{1}{c|}{0.731}          & \multicolumn{1}{c|}{0.746}          & \multicolumn{1}{c|}{0.717}          & \multicolumn{1}{c|}{0.612}          & \multicolumn{1}{c|}{0.627}          & 0.600                               & \multicolumn{1}{c|}{0.453}          & \multicolumn{1}{c|}{0.487}          & \multicolumn{1}{c|}{0.423}          & \multicolumn{1}{c|}{0.360}          & \multicolumn{1}{c|}{0.398}          & \multicolumn{1}{c}{0.352}       \\
TextRNN-Attn  & \multicolumn{1}{c|}{0.743}          & \multicolumn{1}{c|}{0.755}          & \multicolumn{1}{c|}{0.731}          & \multicolumn{1}{c|}{0.625}          & \multicolumn{1}{c|}{0.644}          & 0.611                               & \multicolumn{1}{c|}{0.469}          & \multicolumn{1}{c|}{0.506}          & \multicolumn{1}{c|}{0.438}          & \multicolumn{1}{c|}{0.376}          & \multicolumn{1}{c|}{0.420}          & \multicolumn{1}{c}{0.365}       \\
TextRCNN                  & \multicolumn{1}{c|}{0.739}          & \multicolumn{1}{c|}{0.748}          & \multicolumn{1}{c|}{0.731}          & \multicolumn{1}{c|}{0.620}          & \multicolumn{1}{c|}{0.636}          & 0.612                               & \multicolumn{1}{c|}{0.470}          & \multicolumn{1}{c|}{0.503}          & \multicolumn{1}{c|}{0.442}          & \multicolumn{1}{c|}{0.381}          & \multicolumn{1}{c|}{0.435}          & \multicolumn{1}{c}{0.367}       \\
Transformer               & \multicolumn{1}{c|}{0.718}          & \multicolumn{1}{c|}{0.724}          & \multicolumn{1}{c|}{0.713}          & \multicolumn{1}{c|}{0.597}          & \multicolumn{1}{c|}{0.610}          & 0.590                               & \multicolumn{1}{c|}{0.425}          & \multicolumn{1}{c|}{0.439}          & \multicolumn{1}{c|}{0.411}          & \multicolumn{1}{c|}{0.332}          & \multicolumn{1}{c|}{0.370}          & \multicolumn{1}{c}{0.336}       \\ \hline
HMCN                      & \multicolumn{1}{c|}{0.872}          & \multicolumn{1}{c|}{0.867}          & \multicolumn{1}{c|}{0.878}          & \multicolumn{1}{c|}{0.760}          & \multicolumn{1}{c|}{0.766}          & 0.757                               & \multicolumn{1}{c|}{0.720}          & \multicolumn{1}{c|}{0.740}          & \multicolumn{1}{c|}{0.702}          & \multicolumn{1}{c|}{0.678}          & \multicolumn{1}{c|}{0.744}          & \multicolumn{1}{c}{0.646}       \\
HMCN-R          & \multicolumn{1}{c|}{0.878}          & \multicolumn{1}{c|}{0.887}          & \multicolumn{1}{c|}{0.869}          & \multicolumn{1}{c|}{0.765}          & \multicolumn{1}{c|}{0.773}          & 0.758                               & \multicolumn{1}{c|}{0.677}          & \multicolumn{1}{c|}{0.639}          & \multicolumn{1}{c|}{0.719}          & \multicolumn{1}{c|}{0.609}          & \multicolumn{1}{c|}{0.687}          & \multicolumn{1}{c}{0.565}       \\
HARNN                     & \multicolumn{1}{c|}{0.902}          & \multicolumn{1}{c|}{0.913}          & \multicolumn{1}{c|}{0.891}          & \multicolumn{1}{c|}{0.789}          & \multicolumn{1}{c|}{0.799}          & 0.780                               & \multicolumn{1}{c|}{0.756}          & \multicolumn{1}{c|}{0.796}          & \multicolumn{1}{c|}{0.720}          & \multicolumn{1}{c|}{0.711}          & \multicolumn{1}{c|}{0.779}          & \multicolumn{1}{c}{0.666}       \\ \hline
HMDG-NT     & \multicolumn{1}{c|}{0.889}          & \multicolumn{1}{c|}{0.896}          & \multicolumn{1}{c|}{0.881}          & \multicolumn{1}{c|}{0.774}          & \multicolumn{1}{c|}{0.777}          & 0.772                               & \multicolumn{1}{c|}{0.666}          & \multicolumn{1}{c|}{0.600}          & \multicolumn{1}{c|}{0.749}          & \multicolumn{1}{c|}{0.625}          & \multicolumn{1}{c|}{0.598}          & \multicolumn{1}{c}{0.700}       \\ 
HMDG-NG       & \multicolumn{1}{c|}{\textbf{0.937}} & \multicolumn{1}{c|}{\textbf{0.951}} & \multicolumn{1}{c|}{\underline{0.923}}    & \multicolumn{1}{c|}{\textbf{0.825}} & \multicolumn{1}{c|}{\textbf{0.837}} & \underline{0.813}                         & \multicolumn{1}{c|}{\underline{0.843}}    & \multicolumn{1}{c|}{\underline{0.893}}    & \multicolumn{1}{c|}{\underline{0.798}}    & \multicolumn{1}{c|}{\underline{0.798}}    & \multicolumn{1}{c|}{\textbf{0.869}} & \multicolumn{1}{c}{\underline{0.749}} \\
HMDG       & \multicolumn{1}{l|}{\underline{0.927}}    & \multicolumn{1}{l|}{\underline{0.925}}    & \multicolumn{1}{l|}{\textbf{0.929}} & \multicolumn{1}{l|}{\underline{0.817}}    & \multicolumn{1}{l|}{\underline{0.815}}    & \multicolumn{1}{l|}{\textbf{0.818}} & \multicolumn{1}{l|}{\textbf{0.857}} & \multicolumn{1}{l|}{\textbf{0.896}} & \multicolumn{1}{l|}{\textbf{0.821}} & \multicolumn{1}{l|}{\textbf{0.820}} & \multicolumn{1}{l|}{\underline{0.865}}    & \textbf{0.784}                  \\
\hline
\multirow{3}{*}{Baseline} & \multicolumn{6}{c|}{Level-3}                                                                                                                                                                                                      & \multicolumn{6}{c}{Level-4}                                                                                                                                                                                                   \\ \cline{2-13} 
                          & \multicolumn{3}{c|}{Micro}                                                                                      & \multicolumn{3}{c|}{Macro}                                                                                      & \multicolumn{3}{c|}{Micro}                                                                                      & \multicolumn{3}{c}{Macro}                                                                                   \\ \cline{2-13} 
                          & \multicolumn{1}{c|}{F1}             & \multicolumn{1}{c|}{P}              & \multicolumn{1}{c|}{R}              & \multicolumn{1}{c|}{F1}             & \multicolumn{1}{c|}{P}              & R                                   & \multicolumn{1}{c|}{F1}             & \multicolumn{1}{c|}{P}              & \multicolumn{1}{c|}{R}              & \multicolumn{1}{c|}{F1}             & \multicolumn{1}{c|}{P}              & \multicolumn{1}{c}{R}           \\ \hline
                          TextCNN                   & \multicolumn{1}{l|}{0.330}          & \multicolumn{1}{l|}{0.384}          & \multicolumn{1}{r|}{0.289}          & \multicolumn{1}{r|}{0.209}          & \multicolumn{1}{l|}{0.275}          & \multicolumn{1}{l|}{0.193}          & \multicolumn{1}{l|}{0.153}          & \multicolumn{1}{l|}{0.114}          & \multicolumn{1}{l|}{0.235}          & \multicolumn{1}{l|}{0.112}          & \multicolumn{1}{l|}{0.130}          & 0.134                           \\
DPCNN                     & \multicolumn{1}{l|}{0.225}          & \multicolumn{1}{l|}{0.241}          & \multicolumn{1}{r|}{0.212}          & \multicolumn{1}{r|}{0.145}          & \multicolumn{1}{l|}{0.157}          & \multicolumn{1}{r|}{0.147}          & \multicolumn{1}{r|}{0.083}          & \multicolumn{1}{r|}{0.060}          & \multicolumn{1}{l|}{0.134}          & \multicolumn{1}{l|}{0.055}          & \multicolumn{1}{l|}{0.051}          & 0.077                           \\
FastText                  & \multicolumn{1}{l|}{0.332}          & \multicolumn{1}{l|}{0.373}          & \multicolumn{1}{r|}{0.299}          & \multicolumn{1}{r|}{0.211}          & \multicolumn{1}{l|}{0.260}          & \multicolumn{1}{r|}{0.207}          & \multicolumn{1}{r|}{0.158}          & \multicolumn{1}{r|}{0.116}          & \multicolumn{1}{l|}{0.246}          & \multicolumn{1}{l|}{0.106}          & \multicolumn{1}{l|}{0.114}          & 0.146                           \\


TextRNN                   & \multicolumn{1}{l|}{0.251}          & \multicolumn{1}{l|}{0.293}          & \multicolumn{1}{l|}{0.219}          & \multicolumn{1}{l|}{0.130}          & \multicolumn{1}{l|}{0.159}          & \multicolumn{1}{l|}{0.134}          & \multicolumn{1}{l|}{0.104}          & \multicolumn{1}{l|}{0.077}          & \multicolumn{1}{l|}{0.160}          & \multicolumn{1}{l|}{0.050}          & \multicolumn{1}{l|}{0.053}          & 0.080                           \\
TextRNN-Attn  & \multicolumn{1}{l|}{0.260}          & \multicolumn{1}{l|}{0.306}          & \multicolumn{1}{l|}{0.226}          & \multicolumn{1}{l|}{0.127}          & \multicolumn{1}{l|}{0.160}          & \multicolumn{1}{l|}{0.131}          & \multicolumn{1}{l|}{0.107}          & \multicolumn{1}{l|}{0.079}          & \multicolumn{1}{l|}{0.164}          & \multicolumn{1}{l|}{0.050}          & \multicolumn{1}{l|}{0.055}          & 0.078                           \\
TextRCNN                  & \multicolumn{1}{l|}{0.292}          & \multicolumn{1}{l|}{0.338}          & \multicolumn{1}{l|}{0.257}          & \multicolumn{1}{l|}{0.176}          & \multicolumn{1}{l|}{0.225}          & \multicolumn{1}{l|}{0.171}          & \multicolumn{1}{l|}{0.132}          & \multicolumn{1}{l|}{0.097}          & \multicolumn{1}{l|}{0.202}          & \multicolumn{1}{l|}{0.084}          & \multicolumn{1}{l|}{0.092}          & 0.118                           \\
Transformer               & \multicolumn{1}{l|}{0.204}          & \multicolumn{1}{l|}{0.222}          & \multicolumn{1}{l|}{0.189}          & \multicolumn{1}{l|}{0.112}          & \multicolumn{1}{l|}{0.138}          & \multicolumn{1}{l|}{0.111}          & \multicolumn{1}{l|}{0.073}          & \multicolumn{1}{l|}{0.054}          & \multicolumn{1}{l|}{0.113}          & \multicolumn{1}{l|}{0.037}          & \multicolumn{1}{l|}{0.039}          & 0.051                           \\ \hline
HMCN                      & \multicolumn{1}{l|}{\underline{0.651}}    & \multicolumn{1}{l|}{0.715}          & \multicolumn{1}{l|}{0.598}          & \multicolumn{1}{l|}{\underline{0.566}}    & \multicolumn{1}{l|}{\underline{0.716}}    & \multicolumn{1}{l|}{\underline{0.508}}    & \multicolumn{1}{l|}{\textbf{0.369}} & \multicolumn{1}{l|}{\underline{0.271}}    & \multicolumn{1}{l|}{\underline{0.576}}    & \multicolumn{1}{l|}{\underline{0.350}}    & \multicolumn{1}{l|}{\underline{0.377}}    & \underline{0.435}                     \\
$\text{HMCN-R}$           & \multicolumn{1}{l|}{0.494}          & \multicolumn{1}{l|}{0.434}          & \multicolumn{1}{l|}{0.572}          & \multicolumn{1}{l|}{0.355}          & \multicolumn{1}{l|}{0.311}          & \multicolumn{1}{l|}{0.491}          & \multicolumn{1}{l|}{0.255}          & \multicolumn{1}{l|}{\textbf{0.392}} & \multicolumn{1}{l|}{0.189}          & \multicolumn{1}{l|}{0.206}          & \multicolumn{1}{l|}{0.244}          & 0.252                           \\
HARNN                     & \multicolumn{1}{l|}{0.639}          & \multicolumn{1}{l|}{\underline{0.721}}    & \multicolumn{1}{l|}{0.574}          & \multicolumn{1}{l|}{0.548}          & \multicolumn{1}{l|}{0.690}          & \multicolumn{1}{l|}{0.486}          & \multicolumn{1}{l|}{0.352}          & \multicolumn{1}{l|}{0.260}          & \multicolumn{1}{l|}{0.546}          & \multicolumn{1}{l|}{0.332}          & \multicolumn{1}{l|}{0.352}          & 0.416                           \\ \hline


$\text{HMDG-NT}$      & \multicolumn{1}{l|}{0.275}          & \multicolumn{1}{l|}{0.177}          & \multicolumn{1}{l|}{\underline{0.617}}    & \multicolumn{1}{l|}{0.206}          & \multicolumn{1}{l|}{0.172}          & \multicolumn{1}{l|}{0.428}          & \multicolumn{1}{l|}{0.180}          & \multicolumn{1}{l|}{0.114}          & \multicolumn{1}{l|}{0.431}          & \multicolumn{1}{l|}{0.098}          & \multicolumn{1}{l|}{0.095}          & 0.209                           \\ 
$\text{HMDG-NG}$        & \multicolumn{1}{l|}{0.552}          & \multicolumn{1}{l|}{0.565}          & \multicolumn{1}{l|}{0.540}          & \multicolumn{1}{l|}{0.348}          & \multicolumn{1}{l|}{0.459}          & \multicolumn{1}{l|}{0.337}          & \multicolumn{1}{l|}{0.243}          & \multicolumn{1}{l|}{0.177}          & \multicolumn{1}{l|}{0.386}          & \multicolumn{1}{l|}{0.156}          & \multicolumn{1}{l|}{0.188}          & 0.191                           \\
$\text{HMDG}$        & \multicolumn{1}{l|}{\textbf{0.730}} & \multicolumn{1}{l|}{\textbf{0.801}} & \multicolumn{1}{l|}{\textbf{0.670}} & \multicolumn{1}{l|}{\textbf{0.644}} & \multicolumn{1}{l|}{\textbf{0.766}} & \multicolumn{1}{l|}{\textbf{0.586}} & \multicolumn{1}{l|}{\underline{0.364}}    & \multicolumn{1}{l|}{0.266}          & \multicolumn{1}{l|}{\textbf{0.578}} & \multicolumn{1}{l|}{\textbf{0.375}} & \multicolumn{1}{l|}{\textbf{0.401}} & \textbf{0.449}                  \\
\hline
\end{tabular}%
}


==> document/table/bi.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
% \toprule
\hline
\multicolumn{1}{c|}{\multirow{3}{*}{Baseline}} & \multicolumn{6}{c|}{Level-1}                                                                                                                          & \multicolumn{6}{c}{Level-2}                                                                                                                   \\ \cline{2-13} 
\multicolumn{1}{c|}{}                          & \multicolumn{3}{c|}{Micro}                                                & \multicolumn{3}{c|}{Macro}                                                & \multicolumn{3}{c|}{Micro}                                                & \multicolumn{3}{c}{Macro}                                         \\ \cline{2-13} 
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c|}{P} & \multicolumn{1}{c|}{R} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c|}{P} & \multicolumn{1}{c|}{R} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c|}{P} & \multicolumn{1}{c|}{R} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c|}{P} & R              \\ \hline
TextCNN                                        & 0.739                   & 0.769                  & 0.711                  & 0.627                   & 0.668                  & 0.596                  & 0.485                   & 0.568                  & 0.423                  & 0.400                   & 0.509                  & 0.354          \\
DPCNN                                          & 0.709                   & 0.722                  & 0.696                  & 0.604                   & 0.617                  & 0.596                  & 0.417                   & 0.475                  & 0.371                  & 0.319                   & 0.395                  & 0.294          \\
FastText                                       & 0.739                   & 0.748                  & 0.729                  & 0.631                   & 0.644                  & 0.620                  & 0.487                   & 0.541                  & 0.443                  & 0.401                   & 0.469                  & 0.373          \\

TextRNN                                        & 0.716                   & 0.736                  & 0.697                  & 0.606                   & 0.629                  & 0.588                  & 0.416                   & 0.474                  & 0.370                  & 0.321                   & 0.378                  & 0.298          \\
TextRNN-Attn                                 & 0.723                   & 0.740                  & 0.707                  & 0.611                   & 0.634                  & 0.594                  & 0.422                   & 0.487                  & 0.372                  & 0.325                   & 0.402                  & 0.301          \\
TextRCNN                                       & 0.719                   & 0.739                  & 0.700                  & 0.604                   & 0.638                  & 0.585                  & 0.426                   & 0.489                  & 0.377                  & 0.337                   & 0.402                  & 0.308          \\
Transformer                                    & 0.704                   & 0.686                  & 0.722                  & 0.595                   & 0.578                  & 0.617                  & 0.392                   & 0.396                  & 0.387                  & 0.299                   & 0.331                  & 0.306          \\
\hline
HMCN                                           & 0.841                   & 0.858                  & 0.826                  & 0.735                   & 0.751                  & 0.722                  & 0.626                   & 0.687                  & 0.575                  & 0.546                   & 0.676                  & 0.496          \\
HMCN-R                                       & 0.828                   & 0.831                  & 0.826                  & 0.722                   & 0.725                  & 0.719                  & 0.578                   & 0.655                  & 0.518                  & 0.480                   & 0.587                  & 0.426          \\
HARNN                                          & 0.840                   & 0.839                  & 0.842                  & 0.733                   & 0.731                  & 0.735                  & 0.648                   & 0.702                  & 0.602                  & 0.577                   & 0.660                  & 0.526          \\
\hline

HMDG-NT                                    & 0.821                   & 0.834                  & 0.809                  & 0.715                   & 0.706                  & 0.725                  & 0.554                   & 0.463                  & 0.689                  & 0.492                   & 0.434                  & 0.625          \\

HMDG-NG                                      & \underline{0.876}             & \underline{0.867}            & \underline{0.885}            & \underline{0.772}             & \underline{0.765}         & \underline{0.780}            & \textbf{0.760}             & \textbf{0.812}         & \underline{0.714}            & \textbf{0.700}             & \textbf{0.770}         & \underline{0.651}    \\
HMDG                                       & \textbf{0.881}          & \textbf{0.872}         & \textbf{0.890}         & \textbf{0.776}          & \textbf{0.768}            & \textbf{0.784}         & \underline{0.742}          & \underline{0.756}            & \textbf{0.729}         & \underline{0.680}          & \underline{0.690}            & \textbf{0.679} \\
% \hline
% \midrule
\hline
\multicolumn{1}{c|}{\multirow{3}{*}{Baseline}} & \multicolumn{6}{c|}{Level-3}                                                                                                                          & \multicolumn{6}{c}{Level-4}                                                                                                                   \\ \cline{2-13} 
\multicolumn{1}{c|}{}                          & \multicolumn{3}{c|}{Micro}                                                & \multicolumn{3}{c|}{Macro}                                                & \multicolumn{3}{c|}{Micro}                                                & \multicolumn{3}{c}{Macro}                                         \\ \cline{2-13} 
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c|}{P} & \multicolumn{1}{c|}{R} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c|}{P} & \multicolumn{1}{c|}{R} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c|}{P} & \multicolumn{1}{c|}{R} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c|}{P} & R              \\ \hline
TextCNN                                        & 0.296                   & 0.402                  & 0.234                  & 0.185                   & 0.275                  & 0.160                  & 0.162                   & 0.140                  & 0.192                  & 0.095                   & 0.113                  & 0.111          \\
DPCNN                                          & 0.212                   & 0.286                  & 0.168                  & 0.101                   & 0.144                  & 0.097                  & 0.098                   & 0.084                  & 0.117                  & 0.040                   & 0.049                  & 0.054          \\
FastText                                       & 0.300                   & 0.378                  & 0.248                  & 0.185                   & 0.245                  & 0.173                  & 0.161                   & 0.137                  & 0.196                  & 0.096                   & 0.108                  & 0.117          \\

TextRNN                                        & 0.209                   & 0.283                  & 0.165                  & 0.095                   & 0.126                  & 0.093                  & 0.097                   & 0.084                  & 0.115                  & 0.040                   & 0.045                  & 0.055          \\
TextRNN-Attn                                 & 0.207                   & 0.285                  & 0.162                  & 0.089                   & 0.119                  & 0.088                  & 0.095                   & 0.083                  & 0.112                  & 0.035                   & 0.037                  & 0.052          \\
TextRCNN                                       & 0.236                   & 0.321                  & 0.186                  & 0.123                   & 0.178                  & 0.112                  & 0.123                   & 0.106                  & 0.145                  & 0.059                   & 0.072                  & 0.074          \\
Transformer                                    & 0.175                   & 0.201                  & 0.155                  & 0.090                   & 0.123                  & 0.086                  & 0.070                   & 0.060                  & 0.085                  & 0.025                   & 0.027                  & 0.033          \\
\hline
HMCN                                           & 0.498                   & 0.614                 & 0.419                  & 0.359                   & \underline{0.533}                  & 0.306                  &\underline{0.333}                   & \textbf{0.283}                  & \underline{0.406}                  & \underline{0.243}                   & \underline{0.293}                  & \underline{0.271}          \\
HMCN-R                                       & 0.364                   & 0.496                  & 0.288                  & 0.218                   & 0.344                  & 0.182                  & 0.216                   & 0.186                  & 0.255                  & 0.130                   & 0.168                  & 0.146          \\
HARNN                                          & 0.478                   & 0.578             & 0.407                  & 0.353                   & 0.466                  & 0.310                  & 0.295                   & 0.247                  & 0.366                  & 0.220                   & 0.243                  & 0.253          \\
\hline


HMDG-NT                                    & 0.304                   & 0.220                  & \underline{0.492}                  & 0.201                   & 0.149                  & 0.324                  & 0.204                   & 0.149                  & 0.324                  & 0.104                   & 0.106                  & 0.167          \\ 
HMDG-NG                                      & \underline{0.553}                   & \underline{0.634}                  & 0.491                  & \underline{0.412}                   & 0.530                  &  \underline{0.376}                  & 0.311                   & 0.253                  & 0.404                  & 0.227                   & 0.252                  & 0.269          \\
HMDG                                       & \textbf{0.586}          & \textbf{0.664}         & \textbf{0.525}         & \textbf{0.467}          & \textbf{0.424}         & \textbf{0.576}         & \textbf{0.341}          & \underline{0.273}         & \textbf{0.456}         & \textbf{0.290}          & \textbf{0.330}         & \textbf{0.311} \\\hline
\end{tabular}%
}


==> document/table/differ.tex <==
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{c|llllll|llllll}
\hline
\multirow{3}{*}{Baseline} & \multicolumn{6}{c|}{Level-1}                                                                                                                                                                                         & \multicolumn{6}{c}{Level-2}                                                                                                                                                                                         \\ \cline{2-13} 
                          & \multicolumn{3}{c|}{Micro}                                                                                      & \multicolumn{3}{c|}{Macro}                                                                         & \multicolumn{3}{c|}{Micro}                                                                                      & \multicolumn{3}{c}{Macro}                                                                         \\ \cline{2-13} 
                          & \multicolumn{1}{c|}{F1}             & \multicolumn{1}{c|}{P}              & \multicolumn{1}{c|}{R}              & \multicolumn{1}{c|}{F1}             & \multicolumn{1}{c|}{P}              & \multicolumn{1}{c|}{R} & \multicolumn{1}{c|}{F1}             & \multicolumn{1}{c|}{P}              & \multicolumn{1}{c|}{R}              & \multicolumn{1}{c|}{F1}             & \multicolumn{1}{c|}{P}              & \multicolumn{1}{c}{R} \\ \hline
TextCNN                   & \multicolumn{1}{l|}{0.735}          & \multicolumn{1}{l|}{0.781}          & \multicolumn{1}{l|}{0.694}          & \multicolumn{1}{l|}{0.600}          & \multicolumn{1}{l|}{0.687}          & 0.553                  & \multicolumn{1}{l|}{0.403}          & \multicolumn{1}{l|}{0.538}          & \multicolumn{1}{l|}{0.322}          & \multicolumn{1}{l|}{0.285}          & \multicolumn{1}{l|}{0.417}          & 0.233                 \\
DPCNN                     & \multicolumn{1}{l|}{0.689}          & \multicolumn{1}{l|}{0.705}          & \multicolumn{1}{l|}{0.674}          & \multicolumn{1}{l|}{0.543}          & \multicolumn{1}{l|}{0.592}          & 0.527                  & \multicolumn{1}{l|}{0.284}          & \multicolumn{1}{l|}{0.359}          & \multicolumn{1}{l|}{0.235}          & \multicolumn{1}{l|}{0.151}          & \multicolumn{1}{l|}{0.225}          & 0.137                 \\
FastText                  & \multicolumn{1}{l|}{0.730}          & \multicolumn{1}{l|}{0.741}          & \multicolumn{1}{l|}{0.720}          & \multicolumn{1}{l|}{0.610}          & \multicolumn{1}{l|}{0.628}          & 0.595                  & \multicolumn{1}{l|}{0.402}          & \multicolumn{1}{l|}{0.471}          & \multicolumn{1}{l|}{0.352}          & \multicolumn{1}{l|}{0.303}          & \multicolumn{1}{l|}{0.400}          & 0.263                 \\


TextRNN                   & \multicolumn{1}{l|}{0.692}          & \multicolumn{1}{l|}{0.695}          & \multicolumn{1}{l|}{0.690}          & \multicolumn{1}{l|}{0.569}          & \multicolumn{1}{l|}{0.578}          & 0.562                  & \multicolumn{1}{l|}{0.296}          & \multicolumn{1}{l|}{0.367}          & \multicolumn{1}{l|}{0.249}          & \multicolumn{1}{l|}{0.155}          & \multicolumn{1}{l|}{0.204}          & 0.140                 \\
TextRNN-Attn  & \multicolumn{1}{l|}{0.677}          & \multicolumn{1}{l|}{0.681}          & \multicolumn{1}{l|}{0.673}          & \multicolumn{1}{l|}{0.548}          & \multicolumn{1}{l|}{0.564}          & 0.540                  & \multicolumn{1}{l|}{0.278}          & \multicolumn{1}{l|}{0.335}          & \multicolumn{1}{l|}{0.237}          & \multicolumn{1}{l|}{0.148}          & \multicolumn{1}{l|}{0.173}          & 0.137                 \\
TextRCNN                  & \multicolumn{1}{l|}{0.690}          & \multicolumn{1}{l|}{0.700}          & \multicolumn{1}{l|}{0.680}          & \multicolumn{1}{l|}{0.559}          & \multicolumn{1}{l|}{0.584}          & 0.546                  & \multicolumn{1}{l|}{0.310}          & \multicolumn{1}{l|}{0.407}          & \multicolumn{1}{l|}{0.250}          & \multicolumn{1}{l|}{0.183}          & \multicolumn{1}{l|}{0.272}          & 0.154                 \\
Transformer               & \multicolumn{1}{l|}{0.702}          & \multicolumn{1}{l|}{0.684}          & \multicolumn{1}{l|}{0.721}          & \multicolumn{1}{l|}{0.577}          & \multicolumn{1}{l|}{0.566}          & 0.592                  & \multicolumn{1}{l|}{0.308}          & \multicolumn{1}{l|}{0.325}          & \multicolumn{1}{l|}{0.293}          & \multicolumn{1}{l|}{0.183}          & \multicolumn{1}{l|}{0.221}          & 0.176                 \\ \hline
HMCN                      & \multicolumn{1}{l|}{0.782}          & \multicolumn{1}{l|}{0.794}          & \multicolumn{1}{l|}{0.771}          & \multicolumn{1}{l|}{0.670}          & \multicolumn{1}{l|}{0.687}          & 0.658                  & \multicolumn{1}{l|}{0.565}          & \multicolumn{1}{l|}{0.619}          & \multicolumn{1}{l|}{0.520}          & \multicolumn{1}{l|}{0.461}          & \multicolumn{1}{l|}{0.527}          & 0.429                 \\
HMCN-R          & \multicolumn{1}{l|}{0.770}          & \multicolumn{1}{l|}{0.772}          & \multicolumn{1}{l|}{0.768}          & \multicolumn{1}{l|}{0.664}          & \multicolumn{1}{l|}{0.669}          & 0.664                  & \multicolumn{1}{l|}{0.478}          & \multicolumn{1}{l|}{0.548}          & \multicolumn{1}{l|}{0.425}          & \multicolumn{1}{l|}{0.339}          & \multicolumn{1}{l|}{0.441}          & 0.301                 \\
HARNN                     & \multicolumn{1}{l|}{0.793}          & \multicolumn{1}{l|}{0.796}          & \multicolumn{1}{l|}{0.791}          & \multicolumn{1}{l|}{0.683}          & \multicolumn{1}{l|}{0.697}          & 0.673                  & \multicolumn{1}{l|}{0.529}          & \multicolumn{1}{l|}{0.562}          & \multicolumn{1}{l|}{0.499}          & \multicolumn{1}{l|}{0.409}          & \multicolumn{1}{l|}{0.455}          & 0.386                 \\ \hline


HMDG-NT     & \multicolumn{1}{l|}{0.797}          & \multicolumn{1}{l|}{0.801}          & \multicolumn{1}{l|}{0.793}          & \multicolumn{1}{l|}{0.684}          & \multicolumn{1}{l|}{0.682}          & 0.691                  & \multicolumn{1}{l|}{0.524}          & \multicolumn{1}{l|}{0.495}          & \multicolumn{1}{l|}{0.557}          & \multicolumn{1}{l|}{0.410}          & \multicolumn{1}{l|}{0.412}          & 0.450                 \\ 

HMDG-NG       & \multicolumn{1}{l|}{\underline{0.825}}    & \multicolumn{1}{l|}{\underline{0.828}}    & \multicolumn{1}{l|}{\underline{0.823}}    & \multicolumn{1}{l|}{\underline{0.715}}    & \multicolumn{1}{l|}{\underline{0.717}}    & \underline{0.713}            & \multicolumn{1}{l|}{\underline{0.627}}    & \multicolumn{1}{l|}{\underline{0.634}}    & \multicolumn{1}{l|}{\underline{0.619}}    & \multicolumn{1}{l|}{\underline{0.506}}    & \multicolumn{1}{l|}{\underline{0.533}}    & \textbf{0.610}        \\

HMDG        & \multicolumn{1}{l|}{\textbf{0.835}} & \multicolumn{1}{l|}{\textbf{0.839}} & \multicolumn{1}{l|}{\textbf{0.832}} & \multicolumn{1}{l|}{\textbf{0.719}} & \multicolumn{1}{l|}{\textbf{0.728}} & \textbf{0.715}         & \multicolumn{1}{l|}{\textbf{0.663}} & \multicolumn{1}{l|}{\textbf{0.687}} & \multicolumn{1}{l|}{\textbf{0.642}} & \multicolumn{1}{l|}{\textbf{0.554}} & \multicolumn{1}{l|}{\textbf{0.588}} & \underline{0.540}           \\

\hline
\multirow{3}{*}{Baseline} & \multicolumn{6}{c|}{Level-3}                                                                                                                                                                                         & \multicolumn{6}{c}{Level-4}                                                                                                                                                                                         \\ \cline{2-13} 
                          & \multicolumn{3}{c|}{Micro}                                                                                      & \multicolumn{3}{c|}{Macro}                                                                         & \multicolumn{3}{c|}{Micro}                                                                                      & \multicolumn{3}{c}{Macro}                                                                         \\ \cline{2-13} 
                          & \multicolumn{1}{c|}{F1}             & \multicolumn{1}{c|}{P}              & \multicolumn{1}{c|}{R}              & \multicolumn{1}{c|}{F1}             & \multicolumn{1}{c|}{P}              & \multicolumn{1}{c|}{R} & \multicolumn{1}{c|}{F1}             & \multicolumn{1}{c|}{P}              & \multicolumn{1}{c|}{R}              & \multicolumn{1}{c|}{F1}             & \multicolumn{1}{c|}{P}              & \multicolumn{1}{c}{R} \\ \hline
                          TextCNN                   & \multicolumn{1}{l|}{0.254}          & \multicolumn{1}{l|}{0.366}          & \multicolumn{1}{l|}{0.194}          & \multicolumn{1}{l|}{0.067}          & \multicolumn{1}{l|}{0.099}          & 0.060                  & \multicolumn{1}{l|}{0.190}          & \multicolumn{1}{l|}{0.172}          & \multicolumn{1}{l|}{0.212}          & \multicolumn{1}{l|}{0.040}          & \multicolumn{1}{l|}{0.041}          & 0.052                 \\
DPCNN                     & \multicolumn{1}{l|}{0.132}          & \multicolumn{1}{l|}{0.188}          & \multicolumn{1}{l|}{0.102}          & \multicolumn{1}{l|}{0.017}          & \multicolumn{1}{l|}{0.022}          & 0.017                  & \multicolumn{1}{l|}{0.084}          & \multicolumn{1}{l|}{0.076}          & \multicolumn{1}{l|}{0.095}          & \multicolumn{1}{l|}{0.009}          & \multicolumn{1}{l|}{0.008}          & 0.016                 \\
FastText                  & \multicolumn{1}{l|}{0.251}          & \multicolumn{1}{l|}{0.332}          & \multicolumn{1}{l|}{0.202}          & \multicolumn{1}{l|}{0.078}          & \multicolumn{1}{l|}{0.102}          & 0.070                  & \multicolumn{1}{l|}{0.164}          & \multicolumn{1}{l|}{0.147}          & \multicolumn{1}{l|}{0.185}          & \multicolumn{1}{l|}{0.037}          & \multicolumn{1}{l|}{0.035}          & 0.048                 \\

TextRNN                   & \multicolumn{1}{l|}{0.130}          & \multicolumn{1}{l|}{0.189}          & \multicolumn{1}{l|}{0.100}          & \multicolumn{1}{l|}{0.018}          & \multicolumn{1}{l|}{0.024}          & 0.018                  & \multicolumn{1}{l|}{0.073}          & \multicolumn{1}{l|}{0.066}          & \multicolumn{1}{l|}{0.081}          & \multicolumn{1}{l|}{0.009}          & \multicolumn{1}{l|}{0.009}          & 0.014                 \\
TextRNN-Attn  & \multicolumn{1}{l|}{0.125}          & \multicolumn{1}{l|}{0.176}          & \multicolumn{1}{l|}{0.097}          & \multicolumn{1}{l|}{0.015}          & \multicolumn{1}{l|}{0.017}          & 0.016                  & \multicolumn{1}{l|}{0.071}          & \multicolumn{1}{l|}{0.065}          & \multicolumn{1}{l|}{0.080}          & \multicolumn{1}{l|}{0.008}          & \multicolumn{1}{l|}{0.007}          & 0.014                 \\
TextRCNN                  & \multicolumn{1}{l|}{0.165}          & \multicolumn{1}{l|}{0.242}          & \multicolumn{1}{l|}{0.126}          & \multicolumn{1}{l|}{0.025}          & \multicolumn{1}{l|}{0.032}          & 0.024                  & \multicolumn{1}{l|}{0.105}          & \multicolumn{1}{l|}{0.096}          & \multicolumn{1}{l|}{0.117}          & \multicolumn{1}{l|}{0.010}          & \multicolumn{1}{l|}{0.009}          & 0.019                 \\
Transformer               & \multicolumn{1}{l|}{0.135}          & \multicolumn{1}{l|}{0.184}          & \multicolumn{1}{l|}{0.106}          & \multicolumn{1}{l|}{0.022}          & \multicolumn{1}{l|}{0.033}          & 0.021                  & \multicolumn{1}{l|}{0.070}          & \multicolumn{1}{l|}{0.063}          & \multicolumn{1}{l|}{0.078}          & \multicolumn{1}{l|}{0.009}          & \multicolumn{1}{l|}{0.008}          & 0.014                 \\ \hline
HMCN                      & \multicolumn{1}{l|}{\underline{0.460}}    & \multicolumn{1}{l|}{\underline{0.520}}    & \multicolumn{1}{l|}{0.413}          & \multicolumn{1}{l|}{\underline{0.201}}    & \multicolumn{1}{l|}{\underline{0.241}}    & \underline{0.196}            & \multicolumn{1}{l|}{\underline{0.341}}    & \multicolumn{1}{l|}{\underline{0.297}} & \multicolumn{1}{l|}{\underline{0.401}}    & \multicolumn{1}{l|}{\underline{0.102}}    & \multicolumn{1}{l|}{\underline{0.105}}    & \underline{0.122}           \\
HMCN-R          & \multicolumn{1}{l|}{0.278}          & \multicolumn{1}{l|}{0.221}          & \multicolumn{1}{l|}{0.377}          & \multicolumn{1}{l|}{0.074}          & \multicolumn{1}{l|}{0.099}          & 0.069                  & \multicolumn{1}{l|}{0.183}          & \multicolumn{1}{l|}{0.165} & \multicolumn{1}{l|}{0.205}          & \multicolumn{1}{l|}{0.041}          & \multicolumn{1}{l|}{0.043}          & 0.050                 \\
HARNN                     & \multicolumn{1}{l|}{0.341}          & \multicolumn{1}{l|}{0.398}          & \multicolumn{1}{l|}{0.298}          & \multicolumn{1}{l|}{0.122}          & \multicolumn{1}{l|}{0.147}          & 0.118                  & \multicolumn{1}{l|}{0.226}          & \multicolumn{1}{l|}{0.200}          & \multicolumn{1}{l|}{0.261}          & \multicolumn{1}{l|}{0.058}          & \multicolumn{1}{l|}{0.058}          & 0.072                 \\ \hline
HMDG-NT     & \multicolumn{1}{l|}{0.321}          & \multicolumn{1}{l|}{0.281}          & \multicolumn{1}{l|}{0.372}          & \multicolumn{1}{l|}{0.107}          & \multicolumn{1}{l|}{0.106}          & 0.143                  & \multicolumn{1}{l|}{0.206}          & \multicolumn{1}{l|}{0.161}          & \multicolumn{1}{l|}{0.288}          & \multicolumn{1}{l|}{0.045}          & \multicolumn{1}{l|}{0.043}          & 0.072            

\\
HMDG-NG       & \multicolumn{1}{l|}{0.429}          & \multicolumn{1}{l|}{0.438}          & \multicolumn{1}{l|}{\underline{0.421}}    & \multicolumn{1}{l|}{0.150}          & \multicolumn{1}{l|}{0.167}          & 0.164                  & \multicolumn{1}{l|}{0.281}          & \multicolumn{1}{l|}{0.232}          & \multicolumn{1}{l|}{0.356}          & \multicolumn{1}{l|}{0.075}          & \multicolumn{1}{l|}{0.076}          & 0.100                 \\
HMDG        & \multicolumn{1}{l|}{\textbf{0.536}} & \multicolumn{1}{l|}{\textbf{0.577}} & \multicolumn{1}{l|}{\textbf{0.501}} & \multicolumn{1}{l|}{\textbf{0.239}} & \multicolumn{1}{l|}{\textbf{0.267}} & \textbf{0.241}         & \multicolumn{1}{l|}{\textbf{0.359}} & \multicolumn{1}{l|}{\textbf{0.304}}    & \multicolumn{1}{l|}{\textbf{0.439}} & \multicolumn{1}{l|}{\textbf{0.120}} & \multicolumn{1}{l|}{\textbf{0.119}} & \textbf{0.144}        \\
\hline
\end{tabular}%
}

==> document/table/overall.tex <==
\begin{tabular}{l|c|c|c|c|c|c} 
\hline
Dataset
& \multicolumn{2}{c|}{RP-all}                                   & \multicolumn{2}{c|}{RP-bi}                                    & \multicolumn{2}{c}{RP-differ}                                 \\ 
\hline
      Method
      & \multicolumn{1}{|l|}{Micro-F1} & \multicolumn{1}{|l|}{Macro-F1} & \multicolumn{1}{|l|}{Micro-F1} & \multicolumn{1}{|l|}{Macro-F1} & \multicolumn{1}{|l|}{Micro-F1} & \multicolumn{1}{l}{Macro-F1}  \\ 


\hline
DPCNN         & 0.376                         & 0.108                         & 0.364                         & 0.080                         & 0.346                         & 0.020                         \\
FastText      & 0.460                         & 0.167                         & 0.427                         & 0.149                         & 0.432                         & 0.067                         \\
TextCNN       & 0.456                         & 0.168                         & 0.426                         & 0.148                         & 0.438                         & 0.063                         \\
TextRCNN      & 0.426                         & 0.138                         & 0.381                         & 0.100                         & 0.367                         & 0.025                         \\
$\text{TextRNN}_{attn}$ & 0.413                         & 0.098                         & 0.367                         & 0.072                         & 0.338                         & 0.018                         \\
TextRNN       & 0.402                         & 0.100                         & 0.364                         & 0.077                         & 0.351                         & 0.021                         \\
Transformer   & 0.370                         & 0.083                         & 0.339                         & 0.066                         & 0.358                         & 0.023\\

\hline
$\text{HMCN}$        & 0.676                         & \underline{0.459}                         & \underline{0.582}                         & \underline{0.308}                         & 0.569                         & \underline{0.161}                         \\
$\text{HMCN}_r$      & 0.599                         & 0.289                         & 0.506                         & 0.185                         & 0.478                         & 0.069                         \\
HARNN         & \underline{0.686}                         & 0.443                         & 0.574                         & 0.294                         & 0.516                         & 0.102                         \\ 
\hline


$\text{HMDG}_{flat}$ & 0.436                         & 0.168                         & 0.435                         & 0.164                         & 0.485                         & 0.089                         \\
$\text{HMDG}_{no}$   & 0.668                         & 0.267                         & 0.579                         & 0.242                         & \underline{0.577}                         & 0.127                         \\

$\text{HMDG}_{wg}$   & \textbf{0.748}                         & \textbf{0.512}                         & \textbf{0.648}                         & \textbf{0.384}                         & \textbf{0.624}                         & \textbf{0.190}                         \\
\hline
\end{tabular}


==> style/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> style/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC

